Spindle: Efficient Distributed Training of Multi-Task Large Models via Wavefront Scheduling

Recent foundation models are capable of handling multiple tasks and multiple data modalities with the unified base model structure and several specialized model components. However, efficient training of such multi-task (MT) multi-modal (MM) models poses significant system challenges due to the sophisticated model architecture and the heterogeneous workloads of different tasks and modalities. In this paper, we propose Spindle, a brand new training system tailored for resource-efficient and high-performance training of MT MM models via wavefront scheduling. The key idea of Spindle is to decompose the model execution into waves and address the joint optimization problem sequentially, including both heterogeneity-aware workload parallelization and dependency-driven execution scheduling. We build our system and evaluate it on various MT MM models. Experiments demonstrate the superior performance and efficiency of Spindle, with speedup ratio up to 71% compared to state-of-the-art training systems.

==> Main-Abstract.tex <==
Recent foundation models are capable of handling multiple tasks and multiple data modalities with the unified base model structure and several specialized model components. However, efficient training of such multi-task (MT) multi-modal (MM) models poses significant model management challenges due to the sophisticated model architecture and the heterogeneous workloads of different tasks and modalities.

In this paper, we propose \sname, a brand new training system tailored for resource-efficient and high-performance training of MT MM models.
The key idea of \sname is to decompose the model execution into stages and address the joint optimization problem sequentially, including both heterogeneity-aware workload parallelization and dependency-driven execution scheduling.
We build our system and evaluate it on various MT MM models. 
% Compared with state-of-the-art training systems, \name achieves speedup ratios of up to 71\%.
Experiments demonstrate the superior performance and efficiency of \name, with speedup ratio up to 71\% compared to state-of-the-art training systems.

% Existing training systems are typically optimized for single task training, they lack awareness of the workload heterogeneity and execution dependency, making them inefficient for MT MM models.

% In recent years, deep learning models have achieved remarkable success across various fields. 
% Such advancements have inspired researchers to develop ``generalist models'' — models capable to tackle multiple tasks and multiple modalities within a single unified model, in hopes of moving closer to creating a general-purpose AI. 
% However, efficient training of such sophisticated models poses significant system challenges due to the sophisticated model structure and the diversity and heterogeneity of the tasks and modalities involved. 
% As existing mainstream training systems are typically optimized for single task training, they lack awareness of the heterogeneous scalability and resource demands of various tasks and modalities, making them unsuitable and less effective for generalist models.

% To address this problem, this work develops MTP, a brand new training system tailored for the efficient and scalable multi-task multi-modal training of generalist models.
% First, MTP crafts a series of abstractions for the intricacies of multi-task multi-modal training scenarios, facilitating convenient definition and scheduling of complex multi-modal tasks.
% Second, MTP provides an effective planner that is aware of and adaptive to the heterogeneous workloads of diverse tasks and modalities, delivering efficient resource allocation and training scheduling plan. 
% Moreover, MTP offers a highly efficient runtime framework that supports fine-grained resource allocation at the operator level and flexible management of complex dependencies during the training process. 
% We evaluate MTP in various multi-task multi-modal training scenarios of generalist model. Experiments demonstrate MTP's superior performance and efficiency compared to existing training systems, showcasing its remarkable scalability.
% \red{(Add some data for performance)}


% Compared to state-of-the-art training systems, i.e., Megatron-LM and DeepSpeed, \name achieves speedup ratios of up to 67\% and 71\%, respectively.
% Compared to state-of-the-art training systems, \name achieves speedup ratios of up to 71\%.




\iffalse
Recent foundation models are capable of handling multiple tasks and multiple data modalities with the unified base model structure and several specialized model components. However, efficient training of such multi-task (MT) multi-modal (MM) models poses significant system challenges due to the sophisticated model architecture and the heterogeneous workloads of different tasks and modalities.

In this paper, we propose Spindle, a brand new training system tailored for resource-efficient and high-performance training of MT MM models.
The key idea of Spindle is to decompose the model execution into stages and address the joint optimization problem sequentially, including both heterogeneity-aware workload parallelization and dependency-driven execution scheduling.
We build our system and evaluate it on various MT MM models. 
Experiments demonstrate the superior performance and efficiency of Spindle, with speedup ratio up to 71\% compared to state-of-the-art training systems.


\fi

==> Main-Introduction.tex <==

\iffalse
\section{Introduction}
% \label{sec:intro}

% Deep Learning
% 近几年已经见证了深度学习在众多AI领域中的应用。其中，Transformer-based语言模型~\cite{DBLP:conf/nips/transformer,DBLP:conf/naacl/BERT,gpt1}已经在众多领域中获得了巨大成功，例如自然语言处理领域~\cite{gpt2,DBLP:gpt3,gpt4,DBLP:googleT5,DBLP:llama,DBLP:llama2}，计算机视觉领域~\cite{DBLP:BEiT,DBLP:ViT,DBLP:swin}，音频处理领域~\cite{DBLP:wav2vec2.0,DBLP:whisper,DBLP:speech2text2}，视频分析~\cite{DBLP:VideoMAE,DBLP:ViViT}等。语言模型也推动了多模态学习的发展~\cite{DBLP:CLIP,DBLP:ImageBind,DBLP:BLIP,DBLP:ALBEF,DBLP:CoCa,DBLP:BEIT3,DBLP:BLIP-2,DBLP:PaLM-E,DBLP:MiniGPT-4,DBLP:LLAVA,DBLP:AnyMal}，语言模型的强大理解能力使得模型能够从多个模态中同时学习知识，并对不同模态的信息进行理解和融合，在多模态任务上取得优异性能，例如visual grounding, image captioning。除了在单一任务上取得SOTA性能，最近研究者们开始研究multi-task multi-modal learning~\cite{DBLP:Flamingo, DBLP:GATO,DBLP:UNIFIED-IO,DBLP:OFA,DBLP:OFASys,DBLP:Qwen-VL}，希望能够得到一个generalist models，其能够处理各种不同的多模态任务in an task-agnostic way，以逼近通用人工智能的目标。

Recent years have witnessed the widespread application of deep learning across numerous AI fields. 
Among these, Transformer-based language models~\cite{DBLP:conf/nips/transformer,DBLP:conf/naacl/BERT,gpt1} have achieved significant success in various domains, including natural language processing~\cite{gpt2,DBLP:gpt3,gpt4,DBLP:googleT5,DBLP:llama,DBLP:llama2}, computer vision~\cite{DBLP:BEiT,DBLP:ViT,DBLP:swin}, audio processing~\cite{DBLP:wav2vec2.0,DBLP:whisper,DBLP:speech2text2}, and video analysis~\cite{DBLP:VideoMAE,DBLP:ViViT}, and etc. 
These models have also propelled the advancement of multi-modal learning~\cite{DBLP:CLIP,DBLP:ImageBind,DBLP:BLIP,DBLP:CoCa,DBLP:BEIT3,DBLP:BLIP-2,DBLP:PaLM-E,DBLP:MiniGPT-4,DBLP:LLAVA,DBLP:AnyMAL}, where the robust comprehension abilities of models allow them to learn from and integrate information across different modalities, achieving outstanding performance in multi-modal tasks, such as  visual grounding and image captioning. 
Beyond excelling in singular tasks, recent research has shifted towards exploring multi-task multi-modal learning~\cite{DBLP:Flamingo, DBLP:GATO,DBLP:UNIFIED-IO,DBLP:OFA,DBLP:OFASys,DBLP:Qwen-VL,DBLP:Gemini} with the aim of developing generalist models. These works strive to handle a diverse range of multi-modal tasks in a task-agnostic manner within a single generalist model, moving closer to the goal of achieving artificial general intelligence.

% multi-task multi-modal training related, multi-task important,多列一些multi-task citation，multi-task ablation验证多任务混在一起训练存在的必要性
% 在generalist model的multi-task multi-modal learning过程中，多个任务多种模态的数据被混合在一起训练，在每一个训练iteration中共享模型并同时更新模型，这是当前generalist models普遍采用的训练方法。A generalist model通常由modality encoders和unified encoder组成，前者负责理解和抽取多任务不同模态的特征，后者负责跨模态跨任务特征融合。在训练过程中，不同任务、不同模态之间可能共享和同时更新一部分模型，例如image captioning任务和visual grounding任务共享并同时更新visual encoder模型，audio-related tasks和image-related tasks共享并更新unified encoder模型。与这种混合训练方式相对应的是task-by-task的分阶段训练，每阶段模型只学习single task，但这样训练容易使得模型在处理不同任务的能力上存在偏科，更擅长处理后训练的任务而遗忘部分先训练的任务的能力。我们的empirical observation也证明了这一点。

\iftrue
% \ffc{
A generalist model typically consists of several modality encoders and a unified encoder \red{(Rename one of them? And add a figure here to show various multi-modal tasks activating the need model componem)}, with the former responsible for understanding and extracting features from different modalities across multiple tasks, and the latter for integrating features across modalities and tasks. 
As shown in Figure \red{X}, by routing the inputs through the expected components, we can support various modalities and tasks within one generalist model. 
% Nevertheless, in order to learn such a sophisticated model, it necessiates training with the mixture of data from multiple tasks and modalities. 
A common paradigm to learn such a sophisticated model is by \textit{multi-task multi-modal training}. 
In particular, during each iteration, we use a mixture of data from various tasks and modalities, and the model components are intricately activated and updated by a number of tasks. 
For instance, speech recognition and image captioning tasks shall share the text encoder but feed the visual- and audio-inputs into different encoders. 
% Many empirical results have shown that such a joint training paradigm achieves better model capabilities than performing several single-task training sequentially \red{(cite)}.
Many empirical results have shown that such a joint multi-task training paradigm achieves better multi-modal capabilities for generalist models than performing single-task training separately~\cite{DBLP:Flamingo, DBLP:GATO,DBLP:UNIFIED-IO,DBLP:OFA,DBLP:OFASys,DBLP:Qwen-VL,DBLP:Gemini}.
% }

% \ffc{
Although recent advancements and the explosive growth in model size of language models have driven researchers and engineers to develop notable training systems such as Megatron-LM~\cite{DBLP:megatron} and DeepSpeed~\cite{Deepspeed}, we find that they suffer from extremely poor efficiency when applied to the multi-task multi-modal training of generalist models.   
The reason is that they are mainly designed for single-task training, while lacking optimizations for multi-task multi-modal training.
Specifically, we identify the unique system-level challenges presented by multi-task multi-modal training as follows.
% }
\fi

\iffalse
\old{
{In the multi-task multi-modal learning process of generalist models, data from multiple tasks and modalities are mixed and trained together. 
During each training iteration, the model is shared and updated simultaneously by multiple tasks and modalities. 
Such is a common training paradigm for generalist models in recent works}{~\cite{DBLP:Flamingo, DBLP:GATO,DBLP:UNIFIED-IO,DBLP:OFA,DBLP:OFASys,DBLP:Qwen-VL,DBLP:Gemini}}. 
{A generalist model typically consists of several modality encoders and a unified encoder, with the former responsible for understanding and extracting features from different modalities across multiple tasks, and the latter for integrating features across modalities and tasks. 
Throughout the training process, various tasks and modalities may share and update certain model components, such as image captioning and visual grounding tasks sharing the visual encoder, or audio-related and image-related tasks sharing the unified encoder. 
Such integrated multi-task training paradigm contrasts with task-by-task, continual training, where the model focuses on only a single task at each stage. 
However, in multi-task multi-modal scenario, continual training can lead to imbalances in the model's capability to handle different tasks, more adept at tasks learned later while forgetting those learned earlier. Such limitation is empirically observed in our studies.
}
% The results of this ablation study is not supportive enough, we consider not using it.
% {\red{Here we need an ablation study to show QWen-VAL multi-task learning better than V-A-L continual training.}}
{Therefore, we claim the significance of multi-task multi-modal training when constructing generalist model.}
}






% 经验证据表明增大模型规模能够有效提高模型性能~\cite{DBLP:scaling-laws}，因此，近些年来模型规模不断增大~\cite{gpt2,DBLP:gpt3,gpt4}，模型训练的系统开销也随之不断提高。现代DL系统通常使用多种parallelisms来使用多GPU分布式训练模型。Data parallelism~\cite{DBLP:pytorch-ddp,DBLP:deepspeed-zero}对模型数据进行切分，每个设备负责部分数据的存储和计算。Model parallelism~\cite{DBLP:conf/sc/megatron,DBLP:conf/nips/gpipe,DBLP:conf/sosp/pipedream,pipedream-flush}对模型做切分，各设备负责部分模型的存储和计算。主流的分布式训练系统，such as Megatron-LM~\cite{DBLP:megatron} and DeepSpeed\cite{Deepspeed}，通常混合使用多种parallelisms来高效训练模型，例如Megatron-LM支持3D parallelism，混合使用三种并行范式。more advanced training systems~\cite{DBLP:conf/mlsys/flexflow,DBLP:ALPA,DBLP:Galvatron,Galvatron-BMW} 使用automatic parallelism优化技术来自动探索并行维度的组合。然而，现存的训练系统foucus on single task training中的并行优化，没有针对multi-task multi-modal场景做针对性优化。具体而言，现有系统无法感知不同tasks和modalities对训练资源的不同需求和不同scalability，直接将这些系统apply到generalist model训练场景会导致效率低下。


% current system problem
% Megatron-LM, Deepspeed， focus single task training , however multi-task 
% intro 里可以不提scheduling

\old{
Empirical evidence suggests that increasing model size can effectively improve model performance~\cite{DBLP:scaling-laws}, leading to a trend of growing model sizes in recent years~\cite{gpt2,DBLP:gpt3,gpt4}, alongside rising system overheads for model training. 
Modern deep learning (DL) systems commonly employ various forms of parallelism to enable multi-GPU distributed training. Data parallelism\cite{DBLP:pytorch-ddp,DBLP:deepspeed-zero} divides the input data, with each device responsible for storing and processing a portion of the data. 
Model parallelism~\cite{DBLP:megatron,DBLP:conf/nips/gpipe,DBLP:conf/sosp/pipedream,pipedream-flush} splits the model parameters, assigning parts of the model's storage and computation to different devices. 
Mainstream distributed training systems, such as Megatron-LM~\cite{DBLP:megatron} and DeepSpeed~\cite{Deepspeed}, often combine multiple parallelisms for efficient model training. For instance, Megatron-LM supports 3D parallelism, integrating three types of parallelism paradigms. 
% More advanced training systems~\cite{DBLP:conf/mlsys/flexflow,DBLP:ALPA,DBLP:Galvatron,Galvatron-BMW} utilize automatic parallelism optimization techniques to automatically explore combinations of parallel dimensions.
However, existing training systems focus on parallelism optimization for single-task training and lack targeted optimization for multi-task multi-modal scenarios. 
For instance, current systems do not adapt to the varying demands and scalability of different tasks and modalities, leading to inefficiencies when applied to training generalist models.
}


% 现在我们详细分析multi-task multi-modal training带来的特有的系统层面的挑战。
% (1) Heterogeneity: workload heterogeneity是对generalist model进行multi-task multi-modal training时最显著的挑战。由于复杂的tasks和modalities特性，这种workload heterogeneity既存在于任务间，也存在于任务内。Specifically，不同任务的数据流和激活的模型算子各异，使得任务间负载异构；同一任务不同模态的数据流和激活的模型算子也各不相同，因此任务内算子也存在负载异构。负载异构性使得被不同任务不同模态激活的模型算子，其执行效率随资源规模的scalability各不相同，对资源量的需求也各不相同。直接应用现有训练系统会导致对这种异构性的忽视，从而导致低下的训练效率。
% (2) Dependency：多任务多模态学习中，任务间存在模型依赖，即多任务多模态需共享和更新同一部分模型。同时任务内存在数据流依赖，即任务内不同模态激活的算子存在数据流依赖，即计算拓扑序。这使得我们在设计能感知异构负载的训练系统时，需要兼顾和满足任务间和任务内的dependency。现有系统没有对这种依赖性做特殊处理，使其训练generalist model使无法对多任务多模态做灵活资源分配，例如缺少对多任务模型依赖和同步的支持，使其需要每个设备上都存放模型并执行多任务从而共享模型，而缺少任务内数据流依赖的管理，使其无法在任务内算子间对资源做灵活分配。
% (3) Dynamicity：generalist model的训练过程中，多任务多模态负载可能随着训练进程发生变化，例如某些任务结束训练退出，而某些任务开始加入训练,因此高效的训练系统需要具备对不同任务和模态负载集合自适应的能力。Dynamicity会加剧负载异构性，而现有系统无法对变化的负载做自适应的高效训练。

\old{
Now, we delve into the unique system-level challenges presented by multi-task multi-modal training. 
}
\fi



\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs_intro/intro_observation.pdf}
    \caption{Example of 4 multi-modal tasks of Multitask-CLIP on 16 GPUs. Device utilization comparision of current systems (DeepSpeed) and task-level resource allocation.}
    \label{fig:intro_observation}
\end{figure}

\textbf{Heterogeneity:} First and foremost, a significant challenge in multi-task multi-modal training for generalist models is workload heterogeneity. 
Due to the complex nature of tasks and modalities, such heterogeneity exists both across and within tasks. 
For one thing, different tasks may involve distinct data flows and model components, leading to inter-task workload heterogeneity. 
% \sout{For another, within a single task, different modalities can activate distinct model components, resulting in intra-task workload heterogeneity.}
% \sout{Such heterogeneity causes model components activated by different tasks and modalities to exhibit varying execution efficiency and scalability with respect to resource allocation, leading to diverse resource requirements. 
% Applying existing training systems directly can lead to neglect of such heterogeneity, thereby resulting in poor training efficiency.}
% \ffc{
For another, within a single task, due to the differences in input shapes and model structures, there exists intra-task workload heterogeneity among the processing of different modalities.
As a result, it is essential to allocate suitable amounts of computation resources for diverse model components to strike a balance among them. 
However, existing training systems overlook such workload heterogeneity and usually employ the same resource allocation, leading to poor training efficiency.
% }

\textbf{Dependency:} In multi-task multi-modal training, there exist dependencies among tasks --- as multiple tasks and modalities share certain model components, synchronization is needed before model update. Additionally, there are data flow dependencies within tasks, where components with heterogeneous workloads may depend on each other, forming a computation topology. 
Designing a training system aware of heterogeneous workloads requires accommodating and fulfilling both inter-task and intra-task dependencies. 
% \sout{Current systems lack specialized handling for these dependencies, hampering the ability to allocate resources flexibly in training generalist models. 
% For instance, the lack of support for model dependencies and synchronization across multiple tasks, necessitating that each device holds the model and executes multiple tasks to share the model. 
% Moreover, the absence of management for intra-task data flow dependencies prevents flexible resource allocation among components within a task.}
\ffc{Specifically, when we allocate different amount of resources for the model components to address the challenge of workload heterogeneity, the system should inherently orchestrate the computation logics of each task as well as synchronize multiple tasks sharing the same components.
Nevertheless, current systems fail to take such dependencies into account, making them impractical for efficient multi-task multi-modal training. \red{(Seems a weak conclusion here. Refinement needed.)}
% When running in the distributed manner, they necessitate cumbersome, manual implementations to orchestrate the computation logics of each task as well as to synchronize multiple tasks sharing the same components.
% When we allocate different amount of resources acorss distributed devices to address the workload heterogeneity issue, current systems necessitate cumbersome, manual implementations to orchestrate the computation logics of each task as well as to synchronize multiple tasks sharing the same components.
}

\textbf{Dynamicity:} During the training process of a generalist model, the workloads of tasks and modalities may change dynamically as the training progresses. For example, some tasks may complete and exit the training process, while others may join. Therefore, an efficient training system requires the capability to adapt to the dynamic ensemble of tasks and modalities. Such dynamicity exacerbates workload heterogeneity, and current systems struggle to adapt efficiently to changing workloads.



% we propose MTP, a multi-task ... system. 
% 为了应对以上挑战，在本文中我们提出一个高效的分布式multi-task multi-modal训练系统MTP，其目标是为generalist model提供高效且可扩展性优异的分布式的multi-task multi-modal training。取名自Multi-Task Parallelism，MTP通过为不同任务和模态分配合适的资源量，并细粒度调度多任务进行并行训练，来提高generalist models的分布式训练效率和可扩展性。
% 我们针对该复杂训练场景设计了一套抽象，以Operator为单位细粒度调度任务内模型负载，以Stage为单位管理任务内数据流。我们设计了高效的MTP Planner，其对于不同tasks不同modalities的异构负载具有感知能力自适应性，自动生成高效的多任务多模态资源分配和分布式调度训练方案。同时，我们实现了高效的MTP Runtime Framework，其支持Operator粒度的资源分配和执行，支持灵活的数据流管理和自动的任务间模型同步，MTP基于PyTorch实现，提供了user-friendly的API。我们在常见的generalist model的multi-task multi-modal训练任务上进行了评测，包括Multi-task CLIP, OFASys，QWen-VAL等，实验证明了MTP相比于现有系统的高效性和可扩展性。

To address these challenges, we introduce an efficient distributed multi-task multi-modal training system, MTP. 
Named from Multi-Task Parallelism, MTP allocate appropriate computation resources to various tasks and modalities, finely schedules multi-task parallel training, and provide high efficiency and scalability for multi-task multi-modal training of generalist models.
We first design a set of abstractions tailored for this complex training scenario. Specifically, we schedule the heterogeneous workloads at a granular level with Operators as the unit, and manage data flows by Stages.
We then develop an effective MTP planner, which is aware of and adaptive to the heterogeneous workloads across various tasks and modalities, automatically generating efficient multi-task multi-modal resource allocation and distributed training schedules. 
Moreover, we implement an efficient MTP runtime framework, which supports resource allocation and execution at the granularity of Operators, flexible data flow management, and automatic model synchronization between tasks and modalities. 
MTP is implemented based on PyTorch and offers user-friendly APIs.
Finally, we evaluate MTP on common multi-task multi-modal training scenarios for generalist models. Experiments demonstrated MTP's superior efficiency and scalability compared to existing systems.


% We summurize the contribution of our work as follows:
% (1)	我们深入分析多任务多模态训练场景下的负载特性及系统挑战，并分析了现有系统在多任务多模态训练中的不足。
% (2)	我们提出了一套高效的多任务多模态训练系统MTP，针对该场景设计了一套抽象，以Op为单位细粒度调度任务内模型负载，以Stage为单位管理任务内数据流。
% (3)	MTP提出了一套多任务多模态资源分配调度算法，即MTP Planner，其能够自适应各种多任务多模态负载，细粒度感知负载异构性，并为多任务学习生成高效的分布式调度Plan。
% (4)	MTP基于Torch为多任务多模态学习提供了一套高效MTP Runtime Framework，其支持Op粒度的资源分配和执行，支持灵活的任务数据流管理以应对任务内数据依赖，支持多任务间模型自动同步以应对任务间模型依赖。同时MTP提供了user-friendly的API。
% (5)	我们在常见的多任务多模态负载上做了实验，包括Multi-task CLIP, OFASys，QWen-VAL等，实验验证了MTP相比于现有训练系统的高效性，同时MTP对于集群规模和任务数量具有良好的可扩展性。

We summarize the contributions of our work as follows:

\begin{itemize}[leftmargin=*, nosep]

\item We conduct an in-depth analysis of workload characteristics and system challenges in multi-task multi-modal training and identified limitations in existing systems for such scenarios.

\item We develop MTP, an efficient and scalable multi-task multi-modal training system. MTP introduces a set of abstractions for such complex scenario, scheduling heterogeneous multi-task multi-modal workloads at the granularity of Operators (Ops) and managing task data flows at the Stage level.

\item MTP features a novel MTP Planner, which adapts to various multi-task multi-modal workloads. MTP Planner finely perceives workload heterogeneity and generates efficient resource allocation and distributed scheduling plans for multi-task learning.

\item MTP provides an efficient MTP runtime framework for multi-task multi-modal learning, supporting resource allocation and execution at the granularity of Operators, flexible management of task data flows to address intra-task data dependencies, and automatic synchronization between models across tasks to handle inter-task model dependencies.

\item We evaluate MTP on various multi-task multi-modal scenarios. The experiments demonstrated MTP's efficiency compared to existing training systems, along with its excellent scalability with respect to cluster size and the number of tasks.

\end{itemize}

% Why do we need MTP? 
% MTP is designed for multi-task multi-modal training, where multi-task multi-modal training at the same time, sparsely activate the needed portion of the model. Share the same model, require synchronization between multiple tasks.


% [Significance of multi-task learning]
% Why multi-task learning, rather than continual learning?
% Need an ablation study to show multi-task learning may be superior than continual learning in some cases.

\fi

==> Main-Method-old-5.3.tex <==
% \section{System Design}

\iffalse
\section{Motivation} \label{sec:motivation}
\red{To be written...Maybe motivation and challenge can be illustrated in Introduction?}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{figs/[fake]_4.9_1tasks_16GPUs_mtp.pdf}
%     \caption{\red{[Fake]} For a simple CLIP-LV task, resource re-allocation within an iteration can make better use of GPU resources.}
%     \label{fig:moti-clip}
% \end{figure}

% Why do we need MTP? 
% MTP is designed for multi-task multi-modal training, where multi-task multi-modal training at the same time, sparsely activate the needed portion of the model. Share the same model, require synchronization between multiple tasks.


% [Intro]
% Why multi-task learning, rather than continual learning?
% Need an ablation study to show multi-task learning may be superior than continual learning in some cases.


\subsection{System Challenge of Multi-task Learning}
\begin{itemize}
\item Heterogeneity: Workload heterogeneity among tasks and inside task. Need some profiling results.
\item Dynamicity: Tasks may change dynamically along training.
\item Dependency: Model sharing dependency. Op dependency, operation topological order.
\end{itemize}

Why current system cannot handle these challenges?

What's the difference and relationship between MTP and other lines of work: 

Multi-task multi-modal training system is an unexplored dimension.

Mainstream training system: Megatron-LM Deepspeed

1) Parallelism optimization works, Megatron-LM Deepspeed, MTP multi-task, resource allocation; 

2) Job scheduling works, job are independent, doesn't require model synchronization. These works usually schedule the jobs/tasks at task level, ignoring the heterogeneous workload between the computation Ops inside each task.
\fi


% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{figs/MTP System Framework 4.19.pdf}
%     \caption{\name System Architecture \red{[Sketch for Runtime Engine may be needed?]}}
%     \label{fig:mtp_arch_old}
% \end{figure}

% \zsh{Fig: a stage workflow illustration, including stage[stageOp within], \sflow between stages, and how virtualOp partitioned/instantiated/scheduled/ to several stageOps}
% \zsh{Fig: A System Architecture Illustration (including the whole workflow, from input training tasks, planner's optimization workflow, to real runtime}

\section{\name System Overview}

% MTP是一个高效且可扩展的multi-task multi-modal training framework，其可为generalist models训练中的多任务、多模态提供高效的资源分配和精细的分布式训练调度策略。在该复杂场景中，多个任务和模态共享一个统一的模型，不同的任务或模态会拥有各自的数据流，选择模型的不同通路，激活对应路径上的模型operator并更新对应参数。每一个模型都可由一组数据流和被激活的模型通路表达，不同任务或不同模态间可能共享部分模型算子，并共同更新参数。
% 为了方便地定义和调度复杂的多模态任务，MTP提出了一系列抽象，包括SOp (StageOp), Stage, Dataflow。关于系统架构，\name由\name Planner和\name Runtime Engine组成，其中\name Planner负责分布式资源分配和调度，\name Runtime Engine负责分布式训练runtime。

\name is a highly efficient and scalable multi-task multi-modal training framework designed for the training of generalist models. It facilitates efficient resource allocation and sophisticated distributed training scheduling for multi-task multi-modal training. Within this complex scenario, multiple tasks and modalities share one unified model, where each task or modality operates its own data flow. They select specific pathways within the unified model, activate relevant model operators along these pathways, and update the corresponding parameters. Each multi-modal task can be represented by a set of data flow pathways and the activated model components, with some model operators and parameters potentially shared between different tasks or modalities, requiring simultaneous parameter updates.

\red{need to rewrite overview}

The \name system architecture is illustrated in Figure~\ref{fig:mtp_overview}, consisting of Profiler \& Modeler, Allocator \& Scheduler, and \name Runtime Engine.
Taking user-defined diverse multi-modal tasks as inputs, \name aims to provide the most efficient multi-task multi-modal training on the given GPU cluster.
Firstly, \name Profiler \& Modeler profiles the multi-task multi-modal workloads, and outcomes the scaling curve for each heterogeneous workload, which represents the scaling performance of the workload over computational resources.
Secondly, \name Allocator \& Scheduler allocates the appropriate computational resources for each heterogeneous workload based on its scaling curve, and then schedule the execution of each workload to generate \name stage map, which is organized as multiple \stages and will be illustrated later in \ref{sec:abstraction}.
Finally, given the generated \name stage map, \name runtime engine provides highly efficient distributed training runtime on the GPU cluster.
\red{Here we need to introduce the section organization to match the system architecture.}


% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=\linewidth]{figs/MTP Abstractions 4.19-2.pdf}
%     \caption{\name Abstractions \red{[This figure too detailed, need to reorganize it!]}}
%     \label{fig:mtp_abstraction_old}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figs/MTP-abstraction.pdf}
%     \caption{\name abstractions}
%     \label{fig:mtp_abstraction}
% \end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs_method/MTP Overview.pdf}
    \caption{Architecture overview of \sname.}
    \label{fig:mtp_overview}
\end{figure}

% \section{\name Abstractions} \label{sec:abstraction}
% \red{Here maybe we don't need we give such detailed example for \name abstractions?}

% To conveniently define and schedule the complex multi-modal tasks with heterogeneous workloads, \name introduces a series of abstractions, including \mop, \sop, \sflow and \stage. For the clearer illustration, an example multi-task multi-modal training job is shown in Figure~\ref{fig:mtp_abstraction}, which includes two tasks with different modalities: vision task $T_V$ and audio task $T_A$. Each task activate the needed model components with its own data flow. For instance, $T_V$ activate the vision encoder, text encoder and language model (LM), while $T_A$ activates the audio encoder, text encoder and language model (LM) with its data flow. Now we illustrate the \name abstractions as follows:



% % \begin{itemize}[leftmargin=*]

% % \item \textbf{\mop:} \name defines its most granular scheduling unit as \mop. Different from the common concept of Op (operator) in deep learning, which is usually a bottom-level computation kernel, such as Matmul Op or ReLU Op, \mop in \name allows upper-level and more flexible user-defined scheduling unit. For instance, a \mop in \name can be one Transformer layer, or one ResNet layer. Such upper-level definition enhances user convenience and reduces scheduling complexity.

% % \item \textbf{\mop:} 
% % 为了表征diverse的多任务多模态的异构负载，\name定义了\mop的概念来代表一种unique workload，其对计算资源量有自己unique的scaling curve。每个\mop由模型和数据两部分组成，模型是一连串负载相同或相近的模型层构成的子模型，数据是由某个训练任务激活该部分模型时的数据流。例如，一个vision任务激活24层vision encoder layer构成一个\mop，一个audio任务激活12层audio encoder layer构成另一个\mop 2。即是对于同一个子模型，被不同任务激活会带来不同数据流，从而引起异构负载，例如image captioning任务和visual grounding任务使用不同的数据流激活24层vision encoder layers，构成两个unique \mop。
% % To characterize heterogeneous workloads of diverse multiple tasks and modalities, \name introduces the concept of \mop to represent a unique type of workload. Each \mop has its own scaling curve that uniquely corresponds to its demand on computational resources. A \mop consists of two components: model and data. The former is a sub-module made up of a sequence of model layers with similar or identical workload, and the latter consists of the data flow activated by a specific training task for that model part. For instance, a vision task that activates 24 vision encoder layers constitutes one \mop, while an audio task activating 12 audio encoder layers forms another \mop 2. Even for the same sub-module, different tasks results in different data streams, leading to heterogeneous loads. For example, image captioning task and visual grounding task activate the same sub-module of 24 vision encoder layers with different data flows, resulting in two unique \mops.
% % \subsubsection*{\mop}
% \noindent\textbf{\mop.}
% To characterize heterogeneous workloads of diverse tasks and modalities, \name introduces the concept of \mop, which represents a unique workload characterized by its distinct scalability on computational resources. 
% Each \mop consists of a sub-module—comprising multiple same or similar sequential model layers—and a data flow activated by a specific training task. 
% For instance, in the left side of Figure~\ref{fig:mtp_abstraction_old}, vision task $T_V$ activating 24 vision encoder layers constitutes one \mop, $\operatorname{OP}_{1}$, while audio task $T_A$ activating 12 audio encoder layers forms another, $\operatorname{OP}_{4}$. 
% Even for the same sub-module, different tasks bring heterogeneous workloads due to varying data flows.
% For example, vision task $T_V$ and audio task $T_A$ activate the same sub-module of 12 text encoder layers with different data flows, resulting in two unique \mops, $\operatorname{OP}_{2}$ and $\operatorname{OP}_{5}$.
% % For example, image captioning task and visual grounding task activate the same sub-module of 24 vision encoder layers with different data flows, resulting in two unique \mops.



% % \item \textbf{\sop:} 
% % \subsubsection*{\sop}
% \noindent\textbf{\sop.}
% % 为了管理集群计算资源，\name定义了\sop的概念，每个\sop由多个\mops组成其计算负载，并独占一部分集群设备。例如，一个\sop可以由12层Transformer layers构成，并占据4张GPU卡。\sop的定义是为了更清晰地管理集群资源的分配。
% % Each \sop exclusively occupies a portion of the cluster's hardware for a period of time, owning its execution device group, and is composed of multiple \mops as its computational workload. 
% % To manage cluster computational resources, \name introduces the concept of \sop. 
% % Each \sop is composed of a resource device group and a computational workload. 
% % The device group of each \sop indicates it exclusively occupies a portion of the cluster's hardware for a period of time. 
% % The computational workload of each \sop consists of a portion of layers of a \mop. 
% % Such definition allows to split a \mop to several parts and assign different resource plan flexibly.
% % For instance, for a \mop with 24 encoder layers, we can split it and form two \sops with distinct resource plan, one with 6 layers occupying 4 GPUs, another one with 18 layers occupying 8 GPUs.
% % The definition of \sop is aimed at facilitating a clearer and more flexible allocation of cluster resources.
% To optimize the management of cluster resources, \name introduces \sop, which comprises a resource device group and a computational workload. 
% Specifically, the device group for each \sop indicates it exclusively occupies a segment of the cluster's hardware for a designated period. 
% The computational workload of each \sop consists of selected layers from a \mop, allowing the \mop to be partitioned into multiple sections with adaptable resource allocation. 
% For example, in the right side of Figure~\ref{fig:mtp_abstraction_old} a \mop with 24 vision encoder layers, $\operatorname{OP}_{2}$, can be divided into two \sops: \sop $\operatorname{OP}_{1,1}$ consists of the initial 18 layers using 4 GPUs, while \sop $\operatorname{OP}_{1,2}$ includes the subsequent 6 layers using 2 GPUs. 
% This structure of \sop enhances the clarity and flexibility in distributing cluster resources.

% % \item \textbf{\sflow:} 
% % \subsubsection*{\sflow}
% \noindent\textbf{\sflow.}
% \name introduces \sflow to manage data dependencies between \sops. Each \sflow acts as a conduit between two \sops, facilitating the data transfer from one \sop to the next. 
% Additionally, \sflow orchestrates the transformation of device groups across \sops. 
% For example, \sflow manages the data transfer from \sop $\operatorname{OP}_{1,1}$ on 4 GPUs, to \sop $\operatorname{OP}_{1,2}$ on 8 GPUs during the forward pass, and reverses this flow during the backward pass.

% % \item \textbf{\stage:}
% % \subsubsection*{\stage}
% \noindent\textbf{\stage.}
% % \name用\stage来管理集群资源，每个\stage代表一段时间内对集群资源的管理和分配。具体来说，每个\stage内，\name会将集群设备分配给一部分\sops，这些\sops各自occupy不同device group并行执行，\stage内部的\sops之间不存在数据依赖。为了最大化集群利用效率，\name要求\stage内所有\sops占满集群所有设备并尽可能同时结束。由于multi-task multi-modal异构负载的复杂性，\name允许集群资源分配方案发生变化，\stage也会随之发生切换，\name使用\sflow管理\stage间不同\sops间的数据传输。在\name中，\sop是管理每个负载占用资源的单位，\stage是一段时间内全局集群资源管理的方案。例如Figure右侧展示了8 GPU集群上若干个\name \stage，其中\stage 1由三个位于不同设备上并行执行的\sops组成，分别是来自vision task的占据4 GPUs的18层vision encoder layers和占据2GPUs的12层text encoder layers, 以及来自audio task的占据2GPUs的4 text encoder layers
% \name defines \stage to manage cluster resources globally, with each \stage representing a phase of resource allocation over a specific period. 
% Within each \stage, \name allocates cluster devices to a subset of \sops, each \sop operating on a distinct device group in parallel. 
% There are no data dependencies among the \sops within the same \stage. 
% To maximize cluster efficiency, \name requires that all \sops within a \stage fully utilize all available devices. 
% Given the complexity of heterogeneous multi-task multi-modal workloads, \name allows for changes in resource allocation plans, leading to transitions between \stages. 
% As mentioned, \name employs \sflow to manage data transfer between \sops across different \stages. 
% In \name, a \sop is the unit that manages the resources occupied by each workload, while a \stage represents the scheme for managing global cluster resources over a time period. 
% For example, the right side of Figure~\ref{fig:mtp_abstraction} displays a generated \name Plan organized as several \name \stages on an 8 GPU cluster, where \stage 1 consists of three \sops running in parallel on different devices: 
% $\operatorname{OP}_{1,1}$ occupying 4 GPUs, $\operatorname{OP}_{2,1}$ on 2 GPUs, and $\operatorname{OP}_{4,1}$ using 2 GPUs.
% % \sop $\operatorname{OP}_{1,1}$ occupying 4 GPUs with 18 vision encoder layers and \sop $\operatorname{OP}_{2,1}$ on 2 GPUs with 12 text encoder layers from vision task $T_V$, and \sop $\operatorname{OP}_{1,2}$ from audio task $T_A$ with 4 text encoder layers using 2 GPUs.


% %，每个训练iteration由多个stage串连组成，\name将这种由多个stage组成的训练方案称为\name Plan。\name将复杂的通过stage by stage的forward pass和反过来的backward pass完成一次训练iteration，。例如，Figure右侧展示了8卡两任务的

% % \end{itemize}

\newcommand{\comp}{{(\text{c})}}
\newcommand{\redu}{{(\text{r})}}
\newcommand{\ptp}{{(\text{p})}}
\newcommand{\node}{{(\text{node})}}
\newcommand{\DP}{{(\text{d})}}
\newcommand{\TP}{{(\text{t})}}
\newcommand{\send}{{(\text{s})}}
\newcommand{\recv}{{(\text{r})}}
\newcommand{\dscr}{{(\text{d})}}
\newcommand{\bfa}{\mathbf{a}}

% \section{\name Planner} \label{sec:planner}


% \section{\name Design} \label{sec:system_design}
\section{\name} \label{sec:system_design}
In this section, we introduce the system design of \name. 


\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs_method/MTP Graph Clustering.pdf}
    \caption{\name graph clustering. Diverse multi-modal tasks activate operators and parameters with task-specific data flows, and form the computation graph $\mathcal{G}$. Operators meeting the criteria in \S~\ref{subsec:contraction} will be clustered as a \mop, resulting in the \mop graph $\mathcal{G}_M$. The colors of nodes indicate operator types, e.g., yellow representing the text operator, such as one text encoder layer. 
    % \sout{The background colors indicate different tasks.} 
    The solid arrow lines indicate data flows, while the dotted lines represent the parameters utilized by each operator.}
    \label{fig:graph_cluster}
\end{figure}


\subsection{Graph Contraction} \label{subsec:contraction}
\name interprets diverse multi-modal tasks as a unified directed acyclic computation graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$, where each node $i \in \mathcal{V}$ represents a computational operator and each edge $\langle i,j \rangle \in \mathcal{E}$ denotes the data flow from operator $i$ to $j$. Each task activates specific operators and parameters with unique data flows. 
% \name aims to minimize the execution time of the computation graph $\mathcal{G}$ with appropriate resource allocation and execution schedule for each operator in $\mathcal{G}$. 
% This requires obtaining the computational workload characteristics of each operator. 
% Note that the computation graph usually contains a large amount of operators, while many operators have similar workload characteristics, e.g., the stacked Transformer layers. Therefore, \name first streamline the graph and categorize the diverse operators based on computational workload characteristics by initiating a graph clustering process, as illustrated in Figure~\ref{fig:graph_cluster}. 
\name is designed to minimize the execution time of the computation graph $\mathcal{G}$ by optimizing resource allocation and scheduling for each operator within $\mathcal{G}$. This optimization process necessitates an understanding of the computational workload characteristics for each operator. Given that $\mathcal{G}$ typically includes a large number of operators, many of which share similar workload characteristics (such as stacked Transformer layers), \name initiates a graph clustering process to streamline the complicated graph. It categorizes operators based on their computational workload characteristics, as detailed in Figure~\ref{fig:graph_cluster}.
In this process, operators are clustered into a \mop if they meet the following criteria:

\begin{enumerate}[label=(\arabic*), nosep]
\item There is a data flow between operator $i$ and $j$, i.e.,  $\langle i,j \rangle \in \mathcal{E}$, and both the out-degree of operator $i$ and the in-degree of operator $j$ are 1, ensuring that they are direct predecessors and successors to each other.
\item Operator $i$ and $j$ share the same computational operator type, parameter size, and input data size, confirming identical computational workloads.
\end{enumerate}

During the graph clustering procedure, we traverse the original graph $\mathcal{G}$ in topological order, clustering operators based on the specified criteria until no further pairs of operators meeting these conditions remain. This results in a clustered graph $\mathcal{G}_M = (\mathcal{V}_M, \mathcal{E}_M)$, with each node representing a clustered \mop. Each \mop $m \in \mathcal{V}_M$ consists of $L_m$ consecutive operators from the original graph $\mathcal{G}$, representing a type of unique computation workload.
% that correlates to a group of $\ops$ from the original graph $G$.





% Graph abbreviation / condensation, \mop construction





\subsection{Scalability Estimator} \label{subsec:scale_est}
\sout{Each \mop represents a category of operators, each distinguished by specific workload features. 
The workload features of the \mop is characterized by its resource scalability, which reflects how its execution time varies with changes in resource allocation.
To effectively guide resource allocation and scheduling, \name employs a scalability estimator to accurately capture the resource scalability of each \mop.}
\ffc{As \mops differ in operator types and/or input sizes, they have heterogeneous workloads, necessitating different amount of resources. 
However, there is no doubt that these \mops have distinct resource scalability (i.e., how the execution time varies w.r.t. the amount of allocated resources), posing a significant challenge for resource allocation.
% each \mop has a distinct scalability w.r.t. the amount of allocated resources. 
% , and thus differ in the scalability w.r.t. the amount of allocated resources. 
% Such a diversity in resource scalability poses a significant challenge for resource allocation.
In response to this issue, \name employs a scalability estimator to accurately capture the resource scalability of each \mop.}

For each \mop $m \in \mathcal{G}_M$, we denote its execution time over $n$ GPUs as $T_m(n)$, and its resource scalability as $\varsigma_m(n)=T_m(1)/T_m(n)$, which is the speedup function when the resource allocation expands from $1$ to $n$.
\zsh{The function can be interpreted as speedup, which measures how much \mop accelerates while using more GPUs and can be considered as an indicator of the \textsl{resource scalability} of an \mop~\cite{parallel_gehringer1987_speed_func_def, parallel_hwang1992_speed_func_def, parallel_scheduling_maciej2009}.}
% Different \mops characterizes distinct resource scalability $\varsigma_m(n)$, and the \name scalability estimator aims at estimating the execution time $T_m(n)$, as well as the resource scalability $\varsigma_m(n)$ for each \mop.
% \zsh{and the scalability estimator profiles $T_m(n)$ to estimate the resource scalability $\varsigma_m(n)$ for each \mop.}
As the resource allocation varies, with the total workload evenly distributed across $n$ devices ideally, the workload of \mop $m$ on each device is nearly inversely proportional to $n$.
Our empirical observations indicate that the execution time $T_m(n)$ scales linearly with the workload per device, and $T_m(n)$ can be characterized by a piece-wise linear function with respect to the per device workload, which is inversely proportional to $n$ \zsh{(linear to $1/n$ should revise, showing the probability of uneven distribution on GPUs when $n$ is not a positive factor of [bsz, seqlen, hidden])}:
\begin{equation} \label{eq:fit_curve}
    T_m(n) = \alpha_{m,i} + \frac{\beta_{m,i}}{n},\forall n \in [n_{i-1}, {n_i}], i = 1,\dots,k
\end{equation}
Therefore, our scalability estimator adopts a profiling-simulating combined method to model this function. It begins by profiling several discrete data points $(n_i, T_m(n_i))$ for each \mop. Subsequently, it fits the curve based on Eq.~\ref{eq:fit_curve} to model the execution time $T_m(n)$. Then we calculate resource scalability $\varsigma_m(n)$ to capture the heterogeneous scalability performance of each \mop.

\red{Figure: example of resource scalability curves of \mops.}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{figs_method/Resource Scalability.pdf}
    \caption{An example that resource scalabilities vary among \mops.}
    \label{fig:resrc_scale}
\end{figure}




\subsection{Resource Allocator} \label{subsec:allocator}
In this section, we first describe the definition of the optimization problem (both allocation and scheduling) and dive into the formulation constructed on \mops and $\mathcal{G}_M$.
We then explain how \sname effectively generates bi-point allocations to each \mop.

\subsubsection*{Problem Formulation}
We first formalize the optimization problem on the original computation graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$.
Assume there are $N$ GPUs in total and the computation graph $\mathcal{G}$ is given.
MTP aims to minimize the maximal operator completion time $C$.
We need to find an execution plan $P$, which assigns each operator $i \in \mathcal{V}$ with an \textbf{AS}-tuple $\langle n_i, s_i \rangle \in\mathcal{U}$, such that the operator $i$ is \textbf{A}llocated $n_i$ GPUs and is \textbf{S}cheduled to execute from time $s_i$.
Here the set $\mathcal{U} = \{\langle n, s \rangle | n \in \mathbb{N}, s \geq 0\}$ is formed by all valid AS-tuples.
We can estimate the execution time of operator $i$ as $t_i=T(n_i)$, where $T(\cdot)$ is the execution time function of the corresponding \mop modelled in \S~\ref{subsec:scale_est}.
The optimization problem is formulated as follows:
% \begin{align}
%     \text{Objective: } & \Minimum_{P=\{i:\langle n_i,s_i \rangle | i \in \mathcal{V}, \langle n_i,s_i \rangle \in \mathcal{U}\}} C && \\
%     \text{subject to:} \quad
%     % & t_i = T_i (n_i) && \forall i \in \mathcal{V} \\
%     & C \geq s_i+t_i && \forall i \in \mathcal{V} \\
%     & \sum_{\substack{t \in (s_i, s_i+t_i) \\ i \in \mathcal{V}}} n_i \leq N && \forall t \in \mathbb{R}^+ \label{eq:ori_alloc_capacity}\\
%     & s_i+t_i \leq s_j && \forall \langle i,j \rangle \in \mathcal{E} \label{eq:ori_op_dep}
% \end{align}
\begin{align}
    & \argmin_{P=\{i:\langle n_i,s_i \rangle | i \in \mathcal{V}, \langle n_i,s_i \rangle \in \mathcal{U}\}} C \coloneqq \max_{i \in \mathcal{V}}\{s_i + t_i\} \\
    \text{s.t.} %\quad
    % & t_i = T_i (n_i) && \forall i \in \mathcal{V} \\
    % & C \geq s_i+t_i && \forall i \in \mathcal{V} \\
    & \sum_{{t \in (s_i, s_i+t_i), i \in \mathcal{V}}} n_i \leq N \;\;\; \text{for }\forall t \in \mathbb{R}^+ \label{eq:ori_alloc_capacity}\\
    & s_i+t_i \leq s_j \;\;\; \text{for }\forall \langle i,j \rangle \in \mathcal{E} \label{eq:ori_op_dep}
\end{align}
Here~\eqref{eq:ori_alloc_capacity} is the allocation capacity constraint for any time $t$, and~\eqref{eq:ori_op_dep} is the operator dependency constraint.

To facilitate solving this problem, we leverage the concept of \mop, and re-formulate the problem on the clustered graph $\mathcal{G}_M = (\mathcal{V}_M, \mathcal{E}_M)$.
In this formulation, we split each \mop into different execution part, by assigning it with several ASL-tuples $\langle n,s,l \rangle \in \mathcal{U}_M$, such that $l$ consecutive operators of this \mop type are scheduled to execute from time $s$ with $n$ GPUs.
Here $\mathcal{U}_M = \{\langle n, s, l \rangle | n,l \in \mathbb{N}, s \geq 0\}$ is formed by all valid ASL-tuples.
The optimal execution plan $P$ consists of the sets of ASL-tuples $P_m$ for all \mops.
Given $m \in \mathcal{V}_M$ and $p=\langle n_{m}^{(p)},s_{m}^{(p)},l_{m}^{(p)} \rangle \in P_m$, we denote the execution time span, end time, and time interval by $t_{m}^{(p)} = T_m(n_{m}^{(p)}) \cdot l_{m}^{(p)}$, $e_{m}^{(p)} = s_{m}^{(p)}+t_{m}^{(p)}$, and $I_{m}^{(p)}=(s_{m}^{(p)},e_{m}^{(p)})$, respectively.
Then, the problem is re-written as
% \begin{align}
%     \text{Objective: } & \Minimum_{P=\{m:P_m | m \in \mathcal{V}_M, P_m \subset 2^{\mathcal{U}_M}\}} C && \\
%     \text{Constraints: }
%     % & t_{m}^{(p)} = T_m(n) \cdot l && \forall m \in \mathcal{V}_M, p= \langle n,s,l \rangle  \in P_m \\
%     % & I_m(p) = (s,s+t_{m}^{(p)}) && \forall m \in \mathcal{V}_M, p= \langle n,s,l \rangle \in P_m \\
%     & C \geq e_{m}^{(p)} && \forall m \in \mathcal{V}_M, p \in P_m \\
%     & \sum_{\substack{t\in I_{m}^{(p)} \\ m \in \mathcal{V}_M, p \in P_m}} n_{m}^{(p)} \leq N && \forall t \in \mathbb{R}^+ \label{eq:meta_alloc_capacity} \\
%     & e_{m}^{(p)} \leq s_{j,p'} && \forall \langle m,j \rangle \in \mathcal{E}_M \text{ and} \nonumber \\
%     &&& p \in P_m, p' \in P_j \label{eq:meta_op_dep} \\
%     & I_{m}^{(p_1)} \cap I_{m}^{(p_2)} = \varnothing && \forall m\in \mathcal{V}_M \text{ and} \nonumber \\
%     &&& p_1,p_2\in P_m \label{eq:meta_intraop_dep} \\
%     & \sum_{p \in P_m} l_{m}^{(p)} = L_m && \forall m \in \mathcal{V}_M \label{eq:meta_work_complete}
% \end{align}
\begin{align}
    & \argmin_{P=\{m:P_m | m \in \mathcal{V}_M, P_m \subset 2^{\mathcal{U}_M}\}} C \coloneqq \max_{m \in \mathcal{V}_M, p \in P_m}\{e_{m}^{(p)}\}  \\
    \text{s.t. }
    % & t_{m}^{(p)} = T_m(n) \cdot l && \forall m \in \mathcal{V}_M, p= \langle n,s,l \rangle  \in P_m \\
    % & I_m(p) = (s,s+t_{m}^{(p)}) && \forall m \in \mathcal{V}_M, p= \langle n,s,l \rangle \in P_m \\
    % & C \geq e_{m}^{(p)} \;\;\; \text{for}\;\forall m \in \mathcal{V}_M, p \in P_m \\
    & \sum_{{t\in I_{m}^{(p)}, m \in \mathcal{V}_M, p \in P_m}} n_{m}^{(p)} \leq N \;\;\; \text{for }\forall t \in \mathbb{R}^+ \label{eq:meta_alloc_capacity} \\
    & e_{m}^{(p)} \leq s_{j}^{(p')} \;\;\; \text{for }\forall \langle m,j \rangle \in \mathcal{E}_M, p \in P_m, p' \in P_j \label{eq:meta_op_dep} \\
    & I_{m}^{(p_1)} \cap I_{m}^{(p_2)} = \varnothing \;\;\; \text{for}\;\forall m\in \mathcal{V}_M, p_1,p_2\in P_m \label{eq:meta_intraop_dep} \\
    & \sum_{p \in P_m} l_{m}^{(p)} = L_m \;\;\; \text{for }\forall m \in \mathcal{V}_M \label{eq:meta_work_complete}
\end{align}
The additional constraint~\eqref{eq:meta_intraop_dep} enforces the execution intervals of ASL-tuples in $P_m$ to be pairwise disjoint, because operators within the same \mop cannot execute simultaneously, and \eqref{eq:meta_work_complete} ensures all operators are executed for each \mop.

\red{Subsection: CNTN problem theorem}

\red{Discretized Allocation}
\subsubsection*{Bi-point Discrete Allocation}
If we relax the constraints, allowing GPU resources and operators to be continuously divisible (i.e., $n$ and $l$ in ASL-tuples are real numbers) and removing the operator dependency constraint~\eqref{eq:meta_op_dep}, the problem is transformed into a well-established one \red{(Name of the problem? And use Theorem rather than plain texts here)} in parallel scheduling~\cite{parallel_scheduling_maciej2009}.
Prior theoretical analysis~\cite{pcntn_theory_1981, pcntn_theory_1982} guarantees that the optimal solution, denoted as $\cntnopt$, has the following simple form.
All \mops are started simultaneously, executed all their operators, and finished together.
Formally, each \mop $m$ is assigned a single ASL-tuple $p_m=\langle n_m^\ast, 0, L_m \rangle$, with a uniform end time $e_{m,p_m}=C^\ast$, where $C^\ast$ is the minimum operator completion time.
Leveraging the allocation capacity constraint~\eqref{eq:meta_alloc_capacity}, we obtain the equation
\begin{equation}
    \sum_{m\in \mathcal{V}_M} T_m^\inv\left(\frac{C^\ast}{L_m}\right) = N.
\end{equation}
Our allocator performs a bisection search procedure to solve this equation and obtains the values of $C^\ast$ and all $n_m^\ast$.

To reinstate $n$'s as integers, the allocator separately computes each \mop's proper discrete allocations.
For every \mop $m$, it uses two ASL-tuples $\langle \underline{n_m}, \cdot, \underline{l_m}\rangle, \langle\overline{n_m}, \cdot, \overline{l_m}\rangle$ to fit $\langle n_m^\ast, 0, L_m \rangle$ in $\cntnopt$.
They satisfy two constraints: \zsh{Emphasize this two 'constraints' preserves the 'optimum' property.}
\begin{itemize}[nosep]
    \item Work completion constraint of \mop $m$.
    \begin{equation}\label{eq:bp_dscr_alloc_1}
         L_m = \underline{l_m} + \overline{l_m}.
    \end{equation}
    \item Execution time spans add up to the minimum operator completion time.
    \begin{equation}\label{eq:bp_dscr_alloc_2}
        C^\ast = T_m(\underline{n_m}) \cdot \underline{l_m} + T_m(\overline{n_m}) \cdot \overline{l_m}.
    \end{equation}
\end{itemize}
Here $\underline{n_m}, \overline{n_m}$ are selected as the closest \textsl{valid} integer numbers such that $n_m^\ast \in [\underline{n_m}, \overline{n_m}]$, and $\underline{l_m},\overline{l_m} \in \mathbb{R}^+$ are derived naturally.
%% zsh 4.25
% We impose the \textsl{valid} constraint on the GPU allocation $n$ for $\operatorname{OP}_m$, requiring that $B_m/n$ be an integer thus coincide with the local batch size (or $n=0$ for a dummy allocation).
% We do this for \zsh{three/four reasons}:
% \begin{enumerate}[label=(\arabic*), nosep]
%     \item It is a natural practice in DL training, which avoids the uneven partition of batch size and fully utilize all allocated GPUs.
%     \item It is easy to implement in \sname, which avoids complex logic in P2P communication and potential unnecessary overhead.
%     \item It benefits the process of device placement, lowering the risk of unnecessary inter-node placement, which drastically decreases communication cost.
%     \zsh{\item Tensor parallelism requires structured batch sizes?}
% \end{enumerate}
% wyj
We impose the \textsl{valid} constraint on the allocation $n$ for \mop $m$ for practical reasons, with the constraints as follows:
% requiring that $B_m/n$ be an integer thus coincide with the local batch size (or $n=0$ for a dummy allocation).

% 4.26: allocation n的规整性定义的问题需要讨论，怎么样的n算是规整的n？本质上似乎是需要n能够被所有parallelism degree整除？但是应该是先有n再有并行degree，所以需要n尽量规整才能让并行有更大的空间。我们考虑的gbs B被n整除其实是一种特殊情况：默认全开数据并行，n=dp deg，且gbs B需要被数据并行维度整除，也就是B被n整除，但其实gbs=1, dp=1, tp=2也可以分配两卡。需要讨论如何制定“规整性”概念，不过这里具体规则其实不重要，解法能适应任何规则，只是如何更好地描述这个practical的规整性。

\begin{enumerate}[label=(\arabic*), nosep]
    \item 
    % The allocation $n$ should divide the global batch size $B_m$.
    The allocation $n$ should be divisible by the data parallelism degree. \red{need discussion? avoid global batch size? e.g., gbs=1, dp=1, tp=2, can still be allocated 2 devices?}
    This is a natural practice in distributed training, which avoids the uneven partition of samples and fully utilize all allocated GPUs.
    % \item It is easy to implement in \sname, which avoids complex logic in P2P communication and potential unnecessary overhead.
    \item It benefits the process of device placement, lowering the risk of unnecessary inter-node placement, which drastically decreases communication cost.
    \item \red{How to define the relationship between $n$ and tensor parallelism degree and sequence parallelism degrees?}
\end{enumerate}

The allocator then reinstates $l$'s as integers by rounding $\underline{l_m}, \overline{l_m}$ to their nearest integers.
If an ASL-tuple has an execution time span that is disproportionately small compared to the entirety $C^\ast$, it is removed and its operators are transferred to another tuple of \mop $m$.
This rounding operation preserves the integrity of Eq.~\ref{eq:bp_dscr_alloc_1} and introduces only minor bias to Eq.~\ref{eq:bp_dscr_alloc_2}.

All the processed tuples collectively form the candidate set $\mathcal{S}_{cand}$.
It is worth noting that the allocator only ensures the total execution time span of a \mop is approximately $C^\ast$, and does not specify the start time for each ASL-tuple.

\newcommand{\pqat}{\texttt{PQ\_alloc\_time}\xspace}
\newcommand{\pqnt}{\texttt{PQ\_normt}\xspace}


\begin{figure*}[h] % 双栏跨页，位置选项可以是htb
    \centering
    \begin{subfigure}[b]{0.39\textwidth}
        \includegraphics[width=\textwidth]{figs_method/MTP Device Placement.pdf}
        \caption{\name Device Placement Example.}
        \label{fig:mtp_device_place_1}
    \end{subfigure}
    \hfill % 用于在子图之间添加空白
    \begin{subfigure}[b]{0.59\textwidth} % 宽度设置为文本宽度的48%
        \includegraphics[width=\textwidth]{figs_method/MTP Stage Map.pdf} 
        \caption{\name Execution Plan.}
        \label{fig:mtp_stage_map_1}
    \end{subfigure}
    \caption{Device Placement and \name Execution Plan.}
    % \label{fig:double}
\end{figure*}




\subsection{Stage Scheduler}
In this section, we descirbe how \sname schedules the \mops guided by the allocator output $\setsub{cand}$, and further reinstate the operator dependency constraint by a level-enhanced $\mathcal{G}_M$.

\subsubsection*{Definition of stage}
\sname defines \textsl{\stage} as a unit of scheduling phase.
Within each \stage, \sname allocates all available GPUs to a set of \mops, with each \mop concurrently executing some of its operators using a distinct device group.
The GPU allocations are fixed throughout the entire stage, and the \mops scheduled in the same \stage are not allowed to have data flow dependencies between each other.

\subsubsection*{Stage-greedy Scheduling}
\input{alg_stage_greedy_sched}

\sname performs scheduling stage by stage, as illustrated in Algorithm~\ref{alg:scheduling}.
For a non-scheduled stage $k$ starting at $T_{sched}$, the scheduler first selects ASL-tuples from $\setsub{cand}$ to schedule in this stage, which collectively form the working set $\setsub{work}$ (lines 3-4).
% The stage finishes when any ASL-tuple in $\setsub{work}$ completes the execution of all its operators.
The time span of this stage, denoted as $T_{stage}$, is basically determined by the minimum execution time span among the tuples in $\setsub{work}$.
All tuples in $\setsub{work}$ shed their un-executed operators to align with the minimum execution time span (line 5).
The operators left during this adjustment are scheduled in this stage, while those un-executed form new ASL-tuples.
These two sets of tuples are denoted as $\setsub{sched}$ and $\setsub{unexe}$, respectively.
ASL-tuples in $\setsub{sched}$ may not fully utilize all $N$ available GPUs.
The scheduler thus performs an iterative stage extension procedure if any \mop's allocation $n$ in this stage can be extended to the \mop's next valid allocation number $n'$ (line 6-7).
In the iteration when the ASL-tuple $p$ is extended, additional operators of the same \mop from $\setsub{unexe}$ can be transferred to $p$, making its execution time span to align with $T_{stage}$.
The stage extension procedure concludes when no ASL-tuples in $\setsub{sched}$ can be further extended.
After stage extension, the schedule $\setsub{k}$ in stage $k$ is determined (line 8-9).
The scheduler updates the candidate set and the start time for the next stage (line 10-11).

Stage extension disrupts the equilibrium of Eq.~\eqref{eq:bp_dscr_alloc_2}, ultimately steering the final operator completion time away from the optimal $C^\ast$.
Thus, we carefully devise selection rules for ASL-tuples in working set selection and stage extension to mitigate these losses.

When constructing the working set, the scheduler organizes $\setsub{cand}$ as a priority queue.
It sorts ASL-tuples in descending order, prioritizing the allocation $n$ first and the execution time span $t$ second (line 3).
The primary principle is to schedule ASL-tuples with heavy computational workloads first to minimize their extensions.
This strategy is validated as the discrete allocation, derived from the optimal allocation in $\cntnopt$, effectively serves as a quantitative indicator of the \mop's computation workloads.

In stage-greedy scheduling, if the remaining work across \mops is not balanced, later stages may end up with too few \mops.
This imbalance can lead to resource wastage.
We address this issue in stage extension by reducing the potential imbalances due to prior scheduled stages (including the scheduled part of the current stage).
Specifically, we define the \textsl{normalized remaining time} for \mop $m$ with $l_{remain}$ un-executed operators as follows:
\begin{equation}
    \textsc{NormRT}_m = T_m(n_m^\ast) \cdot l_{remain}.
\end{equation}
Although the execution time for one operator, $T_m(n_m^\ast)$, varies among \mops, each \mop takes the same amount of time, i.e., $C^\ast = T_m(n_m^\ast) \cdot L_m$ to complete the execution of all its operators.
The scheduler greedily selects the ASL-tuple of which the \mop has the largest normalized remaining time for stage extension (line 6).

\subsubsection*{Level-enhanced Operator Dependency}
To deal with the operator dependency in $\mathcal{G}_M$, we assign levels to the \mops, establishing a manually designed order of precedence.
When $\mathcal{G}_M$ is not empty, we pop the \mops from $\mathcal{G}_M$ that have no predecessors and are associated with the smallest level.
\sname generates optimized stage maps for these \mops in a stage-greedy manner, following the workflow described above.



\iffalse
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs_method/MTP Stage Map.pdf}
    \caption{\name stage map, generated by \sname \red{system optimizer}. \zsh{Description needed}}
    \label{fig:mtp_stage_map}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs_method/MTP Device Placement.pdf}
    \caption{\name Device Placement Example.}
    \label{fig:mtp_device_place}
\end{figure}
\fi




\subsection{Device Placement}
The scheduler organizes \mops into multiple consecutive stages, with each \mop allocated a certain amount of cluster resources within each stage. We now discuss how \name determines the specific devices to allocate to each \mop, known as device placement. Device placement mainly affects the communication overhead in \name multi-task multi-modal training. This includes the intra-\mop communication overhead potentially brought about by the distributed parallelism paradigm (e.g., All-Reduce in TP) as well as inter-\mop communication overhead (e.g., transmission costs for data flow between \mops). Below, \name employs several guidelines based on empirical insights or observations to optimize device placement for \mops:


% \red{A figure to illustrate this guidelines for device placement?}
% \zsh{A comparison before/after device placement is needed, showing the communication cost decreases, in an intuitive way}

\subsubsection*{Intra-Device-Island Placement}
Placement within a device island is always preferred for each \mop. 
A device island consists of a group of devices connected by high-bandwidth interconnects (e.g., NVLink, PCIe), typically comprising adjacent devices, such as adjacent GPUs within one node. 
Prioritizing placement within the device island reduces the potential intra-\mop communication costs. 
For example, in a cluster with two GPUs per node, it's more efficient to assign a \mop to a contiguous device group like [0,1] within one node rather than a scattered group like [0,2] across two nodes, as shown in~Figure~\ref{fig:mtp_device_place_1}~(a).
% For example, in a cluster with 4 GPUs per node, it's more efficient to assign a \mop to a contiguous device group like [0,1,2,3] within one node rather than a scattered group like [0,2,4,6] across two nodes.

\subsubsection*{Minimizing Inter-\mop Data Flow Costs}
When two \mops in different stages have a data flow dependency, they should ideally be placed on the same device island to reduce inter-\mop data flow transmission costs leveraging the high intra-island bandwidth. Particularly, when these \mops are allocated the same amount of devices, they should ideally be placed on the exactly same device group, where the data flow may be done via simple copying.
% When two \mops in different stages have a data flow dependency and are allocated the same amount of devices, they should ideally be placed on the same device group to reduce inter-\mop data flow transmission costs. 
For example, if \mop $m$ and \mop $l$ has data flow and are assigned 1 and 2 GPUs, respectively, \name strives to place $m$ on device 1 and $l$ on device 0 and 1~Figure~\ref{fig:mtp_device_place_1}~(b).
This arrangement allows data flow through intra-island communication (i.e., 1 to 0) or intra-device copying (i.e., 1 to 1), avoiding the inter-island communication costs that would occur if $m$ were on device 1 and $l$ on device 2 and 3 on the other node.
% For example, if \mop $m$ and \mop $l$ has data flow and are assigned two GPUs each, \name strives to place them both on [0,1]. 
% This arrangement allows data flow through intra-device copying, avoiding the need for inter-device peer-to-peer (P2P) communication costs that would occur if \mop $m$ were on [0,1] and \mop $l$ on [2,3].

\subsubsection*{Prioritizing High Communication Workloads}
When the ideal scenarios outlined above are not achievable — that is, when it's not possible to place all \mops within the device island or to align all data flows on the same device group — \mops and data flows with higher communication volumes should be prioritized. 
\name estimates the communication volume of each \mop and each data flow to prioritize placing those with higher volumes within a device island and aligning high-volume data flows on the same device group. 
For instance, in~Figure~\ref{fig:mtp_device_place_1}~(c), the transition data flow volume between red \mops and blue \mops are significantly higher than that between yellow ones. Therefore, \name prefer to place the data flow between red and blue \mops within the device island, allowing faster intra-island communication or intra-device copying, while place the data flow between yellow ones across the island. 
This guideline ensures that the most communication-intensive components receive the most efficient hardware configuration to minimize communication overhead.


% old version
% \red{Need re-write, introduce high level idea: \sop pairs with \sflow }
% Until now, our discussion has not addressed P2P communication cost.
% In this section, we explain how, given fixed GPU allocations, we place \mops on GPUs to reduce the P2P communication time between stages.

% We perform the device placement procedure stage by stage, starting from stage $2$.
% Each \mop is assumed to be placed on consecutive GPUs.
% After determining the placement for stage $k-1$, we can order all ATL-tuples by their assigned GPU IDs in a list, denoted as $P_{k-1}$.
% For the next stage $k$, $P_k$ is initially unsorted.
% To organize $P_k$, We sequentially address each position $i$ by testing two types of operations with every $j>i$:
% (1) swapping $P_k[i]$ with $P_k[j]$, and
% (2) inserting $P_k[i]$ into position $j$ and shifting $P_k[i+1]$ to $P_k[j]$ leftward.
% Each operation yields a new placement.
% We select the operation that minimizes the P2P communication time $T^\ptp$ between stage $k-1$ and stage $k$, and advance to the next position, $i+1$.

% \zsh{Experiments show that after optimizing device placement, P2P communication takes up no more than 3\% of the total time in a training iteration.}



% old version MTP design
\iffalse
\section{\name Design} \label{sec:planner}

In this section, we elucidate the optimization workflow of Planner.
% \zsh{
% The abstraction of provided by \sname allows more fine-grained optimization.
% (The granularity: \mop level and malleable \mop)
% }

\red{To revise}
Assume there are $N$ GPUs available and $M$ \mops extracted from all training tasks.
% A GPU can execute at most one \mop at a time.
Every \mop is viewed as a preemptive task, and the GPUs allocated to it can be changed at runtime.
An execution phase is specified by two real numbers: the start time and the duration.
For each \mop, a plan consists of a schedule and corresponding GPU assignments:
the schedule specifies an execution phase within which the \mop is executed,
and the GPU assignments specify the sets of GPUs allocated to this \mop in corresponding execution phases.
The goal is to find a plan for \mops to minimize the training iteration time.

In our configuration, we emphasize two constraints:
\begin{itemize}
    \item \textbf{C. intL}. The number of layers executed in an execution phase for a certain \mop is an integer.
    \item \textbf{C. opDep}. There may exist data flow dependencies among \mops. A \mop can only be scheduled for execution if all of its precedent \mops have already completed their execution.
\end{itemize}

To investigate the overall training time, we divide a complete training iteration into three parts, computation for model forward-backward passes, P2P communication for \sflows between consecutive stages, and synchronization to reduce gradients.
% \zsh{\sout{and synchronization with time $T^\redu$ to reduce gradients (or activations in tensor parallelizem) across GPUs, and finally gradient accumulation factors}}.
Since gradients of all tasks are reduced only once, the reduce time $T^\redu$ becomes less important compared to computation \zsh{take up xx percent? or all baselines have similar reduce time? just a reason}.
Therefore, we mainly optimize computation time $T^\comp$ and P2P communication time $T^\ptp$.
We first construct a plan-to-time model to estimate the computation and communication time of a training iteration given a certain plan (\S~\ref{sec:opt-model}), and generate a close-to-optimal plan in two steps: resource allocation \& scheduling (\S~\ref{sec:opt-alloc}) and device placement (\S~\ref{sec:opt-place}).

Table~\ref{tab:notation} lists notation used in this section, and Algorithm~\ref{alg:opt_workflow} illustrates the optimization workflow.

\begin{table}[tbp]
    \small
    \renewcommand{\arraystretch}{1.25}
    \caption{Notation used in \S~\ref{sec:planner}}
    \label{tab:notation}
    \begin{tabular}{l|p{150pt}}
        \toprule
        \multicolumn{2}{c}{\textbf{Planner Inputs}} \\
        \midrule
        Notation & Description \\ \hline
        $M$ & Number of \mops \\
        $N$ & Number of GPUs \\
        $\operatorname{OP}_m$ & \mop $m$ \\
        $B_m$ & Global batch size of $\operatorname{OP}_m$ \\
        $L_m$ & Number of layers of $\operatorname{OP}_m$ \\
        \midrule
        \multicolumn{2}{c}{\textbf{Planner Outputs}} \\
        \midrule
        $K$ & Number of \stages \\
        $T_k$ & The start time of \stage $k$ \\
        $\operatorname{OP}_{m,k}$ & The \sop instantiated from \mop $m$ in \stage $k$ \\
        $\bfa_{m,k} \in \{0,1\}^N$ & Binary assignment vector indicating the GPUs allocated to $\operatorname{OP}_{m,k}$ \\
        $l_{m,k}$ & Number of layers of $\operatorname{OP}_{m,k}$ \\
        \midrule
        \multicolumn{2}{c}{\textbf{Variables Derived from Planner Outputs}} \\
        \midrule
        $n_{m,k}=\text{sum}(\bfa_{m,k}$) & Number of GPUs allocated to $\operatorname{OP}_{m,k}$ \\
        $b_{m,k}=\left\lceil{B_m}/{n_{m,k}}\right\rceil$ & Local batch size per GPU of $\operatorname{OP}_{m,k}$ \\
        \bottomrule
    \end{tabular}
\end{table}

\input{alg_opt_workflow}

\subsection{Plan-Time Modeling} \label{sec:opt-model}
In this section, we separately model $T^\comp$ for every \mop and $T^\ptp$ for every \sop pair with \sflow.
For simplicity, we omit the subscript $m$ and $(m,k)$.
\red{Maybe find a place to say TP?}

% \subsubsection*{Modeling $T^\comp$}
\subsubsection{Modeling $T^\comp$}
The computation process consists of a forward and a backward pass, and the computation workload is proportional to local batch size $b$.
Consequently, $T^\comp$ scales linearly with $b$ when $b$ is sufficiently large so that computation makes full utilization of GPUs.
For less compute-intensive \mops, we observe different fitting lines for different ranges of $b$.
\zsh{A possible reason is that ...}
Therefore, we model $T^\comp$ for one layer as a piece-wise linear function with $I$ pieces,
\begin{equation}
    T^\comp (B, \bfa) = \alpha_i + \beta_i \cdot b,\forall b \in [b_{i-1}, {b_i}], i = 1,\dots,I,
\end{equation}
where $\alpha_i,\beta_i, (1=)b_0 < b_1 < \cdots < b_I (= B)$ are positive parameters, and the function is continuous when $b=b_i$.
\zsh{(May also include \texttt{all-gather} in SDP.)}

Every \mop is profiled on a single device using a limited set of local batch sizes, because $T^\comp$ is only related to the local batch size $b=\lceil B/n \rceil$ for $n=1,...,N$.
All \mops are profiled in a synchronized manner for a fast and stable profiling process.

% \subsubsection*{Modeling $T^\ptp$}
\subsubsection{Modeling $T^\ptp$}
% For the same \mop, \sname supports dynamic changes in device assignments across different stages.
\sname allows GPU assignment changes across stages, even for the same \mop.
Concurrently, P2P communication is triggered at the stage boundary when there is a \sflow between different \sops.

Due to the large gap between inter-node and intra-node communication bandwidths, we use different parameters for communications within a single node and across nodes.
If we denote send group, receive group and the joint of send/receive groups by $\bfa_s$, $\bfa_r$ and $\hat{\bfa}$ respectively, then $T^\ptp$ can be written as
\begin{equation}
    T^\ptp (B, \bfa_s, \bfa_r) = \left\{
    \begin{array}{ll}
        0 & \bfa_s = \bfa_r \\
        \lambda_i + \mu_i \cdot \max(b_s,b_r) & \hat{\bfa} \in \mathcal{S}_i, i =1,2,
    \end{array}\right.
\end{equation}
where $\mathcal{S}_1=\{\bfa\mid \text{node number of } \bfa=1 \land n\geq 2\}, \mathcal{S}_2 = \{\bfa\mid \text{node number of } \bfa\geq 2\}$, and $\lambda_i, \mu_i$ are positive parameters.

Parameters $\lambda_i$ and $\mu_i$ are solely related to the communication bandwidth between devices and the volume transferred data per sample.
Therefore, we profile the communication bandwidths for different hardware setups offline and derive $T^\ptp$ for each \mop based on the volume of transferred data for an entire local batch.

% \subsubsection*{Modeling $T^\redu$}
% \red{To revise YuJie, my original intention is to include all synchronization (e.g. TP allreduce in forward and backward), except p2p here}
% \zsh{\sout{
% In multi-task multi-modal learning, part of model parameters might be shared by different tasks.
% The parameter cannot do gradient reduction until all related tasks complete their gradient computation on it. [why]
% In \sname, gradient reduction is performed after all \mops finish their backward pass for simplicity.
% }}
% When allocated only one GPU, no synchronization is needed.
% Otherwise, synchronization time is a constant for (sharded) data parallelism since the communication amount is proportional to parameter size, and scales linearly with global batch size $B$ for tensor parallelism since the communication amount is proportional to activation size.

% On the basis of the above considerations,
% \begin{equation}
%     T^\redu (B, \bfa) = \left\{
%     \begin{array}{ll}
%         0 & n = 1 \\
%         \lambda^\redu_i + \mu^\redu_i \cdot b & \bfa \in \mathcal{S}_i, i\in [2],
%     \end{array}\right.
% \end{equation}
% where parameters $\lambda^\redu_i, \mu^\redu_i$ are non-negative and dependent on the parallelism strategy.
% Specifically, $\mu^\redu_i$'s are zeros when the model uses a (sharded) data-parallel strategy.
% \zsh{
% \begin{itemize}
%     \item May add a retrogression factor for straggler/delay, depending on the fitting results.
%     \item Should talk gradient reduction in terms of model parameters, not \mops.
% \end{itemize}
% }

% \subsubsection*{Combining All \stages}
\subsubsection{Combining All \stages}
The time duration of \stage $k$ is the maximum of $T^\comp + T^\ptp$ for all \sops in \stage $k$.
Therefore, combining all \stages together, the total time to be optimized is in the form
\begin{align} \label{eq:t_combine}
\begin{split}
    T = \sum_{k=1}^K \max_{\operatorname{OP}_{m,k} \text{ in \stage $k$}} \{\, & T_m^\comp(B_m, \bfa_{m,k}) \times l_{m,k} \\
    +\, & T_m^\ptp( B_m, \bfa_{m,k-1}, \bfa_{m,k})\,\}.
\end{split}
\end{align}

% $\mathcal{A}_m = \{\bfa_{m,1},\dots,\bfa_{m,K}\}\,\forall m \in [M]$, and $\mathcal{A} = \{\mathcal{A}_1,\dots,\mathcal{A}_M\}$.
% \begin{align}
%     & T = sum_{k=1} \\
%     & \sum_{k=1}^K \max_{m \in M} \left\{ l_{m,k}\times T^\comp(B, \bfa_{m,k}) + T^\ptp( B, \bfa_{m,k}, \bfa_{m,k+1})\right\}.
% \end{align}
% \zsh{Need an integrated form for $T^\redu$ as well.}

% \subsubsection*{Gradient Accumulation}
% The local batch size is typically constrained by the available GPU memory.
% Conversely, the global batch size is optimized for model performance.
% Given a certain number of GPUs, the model may not accommodate within the available GPU memory.
% This issue is particularly noteworthy in multi-task multi-modal learning, where multiple tasks are executed simultaneously.
% Many techniques are proposed to address this issue \tocite.
% Among which, gradient accumulation is an easy yet effective technique.
% It evenly splits the batch into $s$ mini-batches and accumulates gradients $s-1$ rounds locally before a global synchronization and weight update.
% Therefore, for $s$ steps gradient accumulation, the total time of a training iteration is 
% \begin{align}\label{eq:iteration_time}
%     T(B, \mathcal{A}, s) &=
%     s \times T(\lceil B/s \rceil, \mathcal{A}) + \text{Integrated } T^\redu.
% \end{align}

\subsection{Resource Allocation and Scheduling} \label{sec:opt-alloc}
In this section, we focus exclusively on computation time $T^\comp$ by omitting terms $T^\ptp$ in Eq.~\ref{eq:t_combine}.
This simplification allows us to construct the problem in a more manageable and concrete form without the complexities of communication, which we will address in \S~\ref{sec:opt-place}.

% \subsubsection*{Continuous Resource Allocation}
% Suppose the GPU allocation is continuously divisible.
% We further introduce two relaxations:
% (1) Relax \textbf{C. intL}. Each \mop is continuously divisible, meaning that the number of executed layers within an execution phase can be a real number.
% (2) Relax \textbf{C. OpDep}. \mops are independent of each other.

% Define the total work of \mop $m$ as $w_m = E_m(1)$, and the continuous execution speed function \tocite
% % E.F. Gehringer, D.P. Siewiorek, and Z. Segall. Parallel Processing: The Cm� Experience. Digital Press, Bedford, 1987.
% %K. Hwang. Advanced Computer Architecture: Parallelism, Scalability, Programmability. McGraw-Hill, New York, 1993.
% $\varsigma_m(n) = w_m/E_m(n)$ for any real GPU allocation $n \in (0,N]$, and $\varsigma_m(0)=0$.
% It is clear that the workloads
% % \footnote{
% % Here we abuse the term \textsl{work} a little, to represent the amount of computation, for simplicity.
% % In classical parallel scheduling theory, \textsl{work} is represented as the product of the number of resources and processing time.
% % }
% done using $n$ GPUs in time span $t$ is $t \cdot \varsigma_m(n)$.
% \zsh{If rewritten as $\varsigma_m(n)=E_m(1)/E_m(n)$, speed function can be interpreted as speedup, which measures how much application accelerates while using more GPUs and can be considered as an indicator of the application \textsl{scalability}.}

% For non-decreasing speed functions, which is common in practice and also in our case, we introduce set \tocite
% % W¸eglarz, J. (1981). “Project Scheduling with Continuously-Divisible, Doubly Constrained Resources.” Management Science 27, 1040–1052.
% \begin{equation}
%     \mathcal{R} = \left\{ \mathbf{n} = (n_1,\dots,n_M) \middle| n_m \geq 0 \land \sum_{m=1}^M n_m \leq N \right\}
% \end{equation}
% of \textsl{feasible resource allocations} and set
% \begin{equation}
%     \mathcal{U} = \left\{ \mathbf{u} = (u_1,\dots,u_M) \middle| \mathbf{n} \in \mathcal{R} \land u_m=\varsigma_m(n_m) \right\}
% \end{equation}
% of \textsl{feasible transformed resource allocations}.
% Denote $\mathbf{w} = (w_1,\\\dots,w_M)$.
% \begin{theorem}\label{thm:cntn_alloc}\tocite
%     Let $M \leq N$, $\conv(\mathcal{U})$ be the convex hull of the set $\mathcal{U}$, i.e., the set of all convex combinations of the elements of $\mathcal{U}$, and $\mathbf{u} = \mathbf{w}/T$ be a straight line in the space of transformed resource allocations given by the parametric equations $u_m=w_m/T, m\in [M]$.
%     Then the minimum makespan value for the continuous resource allocation problem can be found from
%     \begin{equation}
%         T^\ast = \min \left\{ T \mid T>0 \land \mathbf{w}/T \in\conv(\mathcal{U})\right\}.
%     \end{equation}
% \end{theorem}
% % W¸eglarz, J. (1981). “Project Scheduling with Continuously-Divisible, Doubly Constrained Resources.” Management Science 27, 1040–1052.
% % W¸eglarz, J. (1982). “Modelling and Control of Dynamic Resource Allocation Project Scheduling Systems.” In S.G. Tzafestas (ed.), Optimization and Control of Dynamic Operational Research Models. Amsterdam: North-Holland.
% Here \textsl{makespan} means the maximum of \mop completion time.
% Theorem \ref{thm:cntn_alloc} states that the optimal solution $(T^\ast,\mathbf{u}^\ast)$ corresponds to the intersection point of $\mathbf{u}=\mathbf{w}/T\,(T > 0)$ and the boundary of $\conv(\mathcal{U})$.

% \subsubsection*{From Continuous to Discrete}
% For the discrete problem, only integer allocations are allowed, and the speed functions, denoted $\varsigma^\dscr$, are initially defined only for integer allocations.
% By extending $\varsigma^\dscr$ to a piecewise linear function $\varsigma$ defined over $\mathbb{R}$, we can establish meaningful connections between the discrete problem and its continuous variation.
% It can be proved that the minimum makespan of the discrete problem is equivalent to that of its continuous counterpart.
% Furthermore, if $F^\ast$ is defined as the facet of convex polytope $\conv(\mathcal{U})$ such that the optimal point $\mathbf{u}^\ast \in F^\ast$, then $\mathbf{u}^\ast$ can be represented as a convex combination of the vertices of $F^\ast$.
% From this representation, we can generate an optimal discrete plan through the vertices and their coefficients in the convex combination, as each vertex corresponds to a valid discrete GPU allocation \tocite.
% % J. Blazewicz, M.Y. Kovalyov, M. Machowiak, D. Trystram, and J. Weglarz, “Malleable Task Scheduling to Minimize the Makespan,” Annals of Operations Research, vol. 129, pp. 65-80, 2004.
% \zsh{Detailed proofs are provided in Appendix or refer to reference.}

% To find the optimal solution $(T^\ast, \mathbf{u}^\ast)$ to the continuous problem, we need to consider the equation
% \begin{equation}
%     \sum_{m=1}^M \varsigma^\inv_m(w_m/T) = N,
% \end{equation}
% where $\varsigma^\inv_m$ is the inverse function of $\varsigma_m$.
% It is straightforward to perform a bisection search to solve the equation.
% We illustrate details in Algorithm~\ref{alg:bisection_search} in Appendix.
% The essential difficulty to the discrete problem is how to determine the facet $F^\ast$ and find the convex combination, since the vertices with positive coefficients in the convex combination directly relate to the optimal discrete plan.
% The discrete problem when speed functions are all convex or all concave has been studied \tocite, with a complexity guarantee of $\mathop{O}(M)$ and $\mathop{O}(M\max\{N,M \log^2 N\})$, respectively.
% % May not cite these references:
% % J. Blazewicz, M.Y. Kovalyov, M. Machowiak, D. Trystram, and J. Weglarz, “Malleable Task Scheduling to Minimize the Makespan,” Annals of Operations Research, vol. 129, pp. 65-80, 2004.
% % Jacek Blazewicz, Mikhail Y. Kovalyov, Maciej Machowiak, Denis Trystram, and Jan WeglarzPreemptable, "Malleable Task Scheduling Problem"
% However, for arbitrary non-decreasing speed functions, the effective algorithm remains unknown.
% The best guarantee of time is $\mathop{O}((N+1)^{3M-3})$, which is unacceptable in our case where $N,M$ can be larger than $10$.

% % \subsubsection*{Technical Background}
% \subsubsection{Technical Background}
% We initiate our discussion by removing the two constraints, \textbf{C. intL} and \textbf{C. opDep}, transforming the problem into a well-established one in parallel scheduling~\cite{parallel_scheduling_maciej2009}.

% Note that for a certain \mop $\operatorname{OP}_m$, $B_m$ and $L_m$ are fixed, we can denote the total execution time of $L_m$ layers \mop $m$ for an assignment $\bfa$ with $n$ GPUs by $E_m(n) \coloneq T^\comp_m (B_m,\bfa) \cdot L_m$.
% The total workload is represented as $w_m = E_m(1)$, and the non-decreasing speed function is $\varsigma_m(n)=w_m/E_m(n)$ for any GPU allocation $n>0$ and $\varsigma_m(0)=0$, as is defined in previous research~\cite{parallel_gehringer1987_speed_func_def, parallel_hwang1992_speed_func_def}.
% The workload completed using $n$ GPUs over a time span $t$ equals $t\cdot \varsigma_m(n)$.
% % \zsh{\sout{If rewritten as $\varsigma_m(n)=E_m(1)/E_m(n)$, speed function can be interpreted as speedup, which measures how much application accelerates while using more GPUs and can be considered as an indicator of the application \textsl{scalability}}.}

% Previous work~\cite{Blazewicz2004SchedulingMT_convex, Blazewicz2006SchedulingPMT_concave} has demonstrated efficient solution algorithm when speed functions are either all convex or all concave.
% % \zsh{\sout{, with a complexity guarantee of $O(M)$ and $O(M \max\{N, M\log^2 N\})$, respectively.}}
% However, for arbitrary non-decreasing speed functions, the best-known time complexity of the solution algorithm is $O((N+1)^{3M-3})$~\cite{Blazewicz2004SchedulingMT_convex}, which is impractical in our case where $N,M$ can exceed $10$.

% If we further assume GPU resources are continuously divisible (i.e., allocation $n$ is a real number), the optimal solution for this problem, denoted as $\cntnopt$, has a simple form~\cite{pcntn_theory_1981, pcntn_theory_1982}:
% each $\operatorname{OP}_m$ is scheduled within the same execution phase $[0, T^\ast]$ and is allocated $n_m^\ast$ GPUs.
% Here $T^\ast$ is the minimum makespan, and the sum of all allocations $n_m^\ast$ equals $N$.

% % \subsubsection*{Bi-point Discrete Allocation}
% \subsubsection{Bi-point Discrete Allocation}
% In our case, it can be verified that the speed function $\varsigma$, due to the term $b=\lceil B/n \rceil$, is not concave nor convex.
% To resolve this issue, we separately compute each \mop's proper discrete allocations.
% For every $\operatorname{OP}_m$, we use two discrete allocation-time pairs $(\underline{n_m}, \underline{t_m}), (\overline{n_m}, \overline{t_m})$ to fit $(n_m^\ast, T^\ast)$ in $\cntnopt$.
% They satisfy two constraints:
% \begin{itemize}
%     \item Integrated workload equals the total workload.
%     \begin{equation}\label{eq:bipoint_dscr_alloc_1}
%         \underline{t_m} \cdot \varsigma_m(\underline{n_m}) + \overline{t_m} \cdot \varsigma_m(\overline{n_m}) = w_m.
%     \end{equation}
%     \item Scheduled time lengths add up to the minimum makespan.
%     \begin{equation}\label{eq:bipoint_dscr_alloc_2}
%         \underline{t_m}+\overline{t_m}=T^\ast.
%     \end{equation}
% \end{itemize}
% Here $\underline{n_m}, \overline{n_m}$ are selected as the closest \textsl{valid} integer numbers such that $n_m^\ast \in [\underline{n_m}, \overline{n_m}]$, and $\underline{t_m},\overline{t_m}$ are derived naturally.
% We impose the \textsl{valid} constraint on the GPU allocation $n$ for $\operatorname{OP}_m$, requiring that $B_m/n$ be an integer thus coincide with the local batch size (or $n=0$ for a dummy allocation).
% We do this for \zsh{three/four reasons}:
% \begin{itemize}
%     \item It is a natural practice in DL training, which avoids the uneven partition of batch size and fully utilize all allocated GPUs.
%     \item It is easy to implement in \sname, which avoids complex logic in P2P communication and potential unnecessary overhead.
%     \item It benefits the GPU assignment process, lowering the risk of unnecessary inter-node placement, which drastically decreases communication cost.
%     \zsh{\item Tensor parallelism requires structured batch sizes?}
% \end{itemize}

% \newcommand{\pqat}{\texttt{PQ\_alloc\_time}\xspace}
% \newcommand{\pqnt}{\texttt{PQ\_normt}\xspace}

% \subsubsection*{Stage-greedy Scheduling}
\subsubsection{Stage-greedy Scheduling}
Guided by previously generated discrete allocation-time pairs, we employ a stage-greedy procedure to schedule all \mops.
In this procedure, we reinstate the constraint \textbf{C. intL} and perform scheduling over the number of layers instead of execution time.
The procedure is illustrated in Algorithm~\ref{alg:scheduling}.

First, we label each allocation-time pair $(n,t)$ of $\operatorname{OP}_m$ with the number of executed layers $l$, and round $l$ to the nearest integer $l'$, along with its execution time, together form an ATL-tuple $(\operatorname{OP}_m, (n,t',l'))$.
If the time of an ATL-tuple $(\operatorname{OP}_m, (n,t,l))$ is disproportionately small compared to the entirety, we remove the tuple and transfer its layers to $\operatorname{OP}_m$'s another tuple.
All the processed tuples collectively form the candidate set $\mathcal{S}_{cand}$.

Next, we start scheduling stage by stage.
To begin with, We construct two priority queues, \pqat and \pqnt, each containing some ATL-tuples.
We will discuss their design intentions after reviewing the algorithm workflow for brevity and clarity.
Now for an empty stage with a determined start time $T_{sched}$, \pqat contains ATL-tuples in $\mathcal{S}_{cand}$.
We construct a working set $\mathcal{S}_{work}$, in such a way that we successively select tuples popped from \pqat, discarding those with repeated \mops, until the remaining $N_{remain}$ GPUs cannot accommodate the next tuple.
The span of this stage, denoted as $T_{stage}$, is determined by the shortest time span among the tuples in $\mathcal{S}_{work}$.
All tuples in $\mathcal{S}_{work}$ shed their excess layers to align with $T_{stage}$.
The layers left during this adjustment are scheduled in this stage, while those removed formulate new tuples.
These two sets of tuples are denoted $\setsub{sched}$ and $\setsub{excess}$, respectively.
Then we perform an iterative stage extension procedure if any \mop's allocation in this stage can be extended.
\pqnt contains all ATL-tuples in $\mathcal{S}_{excess}$.
For each iteration, we select the first satisfied tuple $(\operatorname{OP}_m,(n_0,t_0,l_0))$ popped from \pqnt such that $\operatorname{OP}_m$'s scheduled tuple $(\operatorname{OP}_m,(n,t,l))$ in this stage can increase the GPU allocation $n$ to $\operatorname{OP}_m$'s next valid allocation number $n'$ while the total number of allocated GPUs does not exceed $N$.
We extend the tuple $(\operatorname{OP}_m,(n,t,l))$ to $(\operatorname{OP}_m,(n',t',l+l'))$ with $l'$ layers from $(\operatorname{OP}_m,(n_0,t_0,l_0))$ and make sure $t'$ not exceed $T_{stage}$.
The remaining part, $(\operatorname{OP}_m,(n_0,t_0',l_0-l'))$, are again pushed into \pqnt.
After stage extension, the scheduling for this stage is complete.
The start time for next stage will be updated to $T_{sched}+T_{stage}$.

Stage extension disrupts the equilibrium of the equation system of Eq.~\ref{eq:bipoint_dscr_alloc_1} and Eq.~\ref{eq:bipoint_dscr_alloc_2}, ultimately steering the final makespan away from the optimal $T^\ast$.
Thus, we carefully select sorting rules in \pqnt and \pqat is to mitigate the losses incurred by stage extension.

In $\cntnopt$, $\operatorname{OP}_m$'s allocation $n_m^\ast$ can be interpreted as a quantitative indicator of the computation load for $\operatorname{OP}_m$.
Therefore, high values of $n$ and $t$ in an ATL-tuple, which derived from the optimal allocation, suggest a heavy computation load.
Given that the losses incurred by extensions on these tuples' allocations are substantial, we sort ATL-tuples $(\operatorname{OP}_m,(n,t,l))$ in \pqat in descending order, prioritizing $n$ first and $t$ second.
Scheduling these tuples first helps to reduce the likelihood of needing extensions on their allocations.

When performing stage extension, it is critical to adjust for the biases of remaining workload across \mops caused by prior scheduled stages (including the scheduled part of the current stage).
Inspired by this, we define the \textsl{normalized time} for \mop $m$ with workload $w$ (not necessarily equals $w_m$) as follows:
\begin{equation}
    \normt_m(w) = \frac{w}{\varsigma_m(n_m^\ast)}.
\end{equation}
Here $\varsigma_m(n_m^\ast)$ is the normalized speed for $\operatorname{OP}_m$.
Although the total workload $w_m$ varies from \mop to \mop, each \mop takes the same amount of time, i.e., $T^\ast=w_m/\varsigma_m(n_m^\ast)=\normt_m(w_m)$ to complete computation with the normalized speed.
Thus, normalized time is a fair metric to assess the relative workloads across \mops.
We sort the tuples $(\operatorname{OP}_m,(n_0,t_0,l_0))$ in \pqnt by the normalized time of the remaining workloads for $\operatorname{OP}_m$, in descending order.

\input{alg_stage_greedy_sched}

% \subsubsection*{Level-enhanced \mop DAG}
\subsubsection{Level-enhanced \mop DAG}
To deal with \textbf{C. opDep}, we initially construct a directed acyclic graph (DAG), denoted as $G$, with \mops as nodes and data flow dependencies as edges.
We then assign levels to the \mops, establishing a manually designed order of precedence.
When $G$ is not empty, we pop the \mops from $G$ that have no predecessors and are associated with the smallest level.
We generate plans for these \mops, following the workflow described above.




\subsection{Device Placement} \label{sec:opt-place}
\red{Need re-write, introduce high level idea: \sop pairs with \sflow }
Until now, our discussion has not addressed P2P communication cost.
In this section, we explain how, given fixed GPU allocations, we place \mops on GPUs to reduce the P2P communication time between stages.

We perform the device placement procedure stage by stage, starting from stage $2$.
Each \mop is assumed to be placed on consecutive GPUs.
After determining the placement for stage $k-1$, we can order all ATL-tuples by their assigned GPU IDs in a list, denoted as $P_{k-1}$.
For the next stage $k$, $P_k$ is initially unsorted.
To organize $P_k$, We sequentially address each position $i$ by testing two types of operations with every $j>i$:
(1) swapping $P_k[i]$ with $P_k[j]$, and
(2) inserting $P_k[i]$ into position $j$ and shifting $P_k[i+1]$ to $P_k[j]$ leftward.
Each operation yields a new placement.
We select the operation that minimizes the P2P communication time $T^\ptp$ between stage $k-1$ and stage $k$, and advance to the next position, $i+1$.

\zsh{Experiments show that after optimizing device placement, P2P communication takes up no more than 3\% of the total time in a training iteration.}

% \subsection{Parallelism Optimization}

% How to cooperate with Galvatron?


\fi





==> alg_opt_workflow.tex <==

\begin{algorithm}[t]
    \caption{Planner Optimization Workflow}
    \label{alg:opt_workflow}
    \scalebox{0.92}{
    \begin{minipage}{\textwidth}
    \LinesNumbered
    \DontPrintSemicolon
        \KwIn{\# GPUs $N$, \mops $\mathcal{C}:\{\op_m\}_{m=1}^M$}
        \KwOut{
            optimized training iteration time $T$, \\
            \quad\quad\quad\quad plan for all stages $P:\{P_k\}_{k=1}^K$
        }
        Do trial runs and plan-time modeling for all \mops.\;
        $\{(\operatorname{OP}_m, \text{level}_m)\}_{m=1}^M \gets \texttt{Assign\_Op\_Level}(\mathcal{C})$  \tcp*[h]{optional}\;
        $G \gets \texttt{Construct\_Level\_DAG}(\{(\op_m, \text{level}_m)\}_{m=1}^M)$\;
        $T, P \gets 0, \varnothing$\;
        \While{$G$ is not empty}{
            $\setsub{cand\_op} \gets G.\texttt{pop\_valid}()$\;
            $P_{CNTN} \gets \texttt{Solve\_CNTN\_Problem}(N, \setsub{cand\_op})$\;
            $\setsub{cand} \gets \texttt{Bipoint\_DSCR\_Alloc}(P_{CNTN})$\;
            $P_{DSCR}, T \gets \texttt{Stage\_Greedy\_Sched}(N, T, \setsub{cand})$\;
            $P.\texttt{extend}(P_{DSCR})$\;
        }
        \ForEach{plan $P_k$ of stage $k\geq 2$ in $P$}{
            $P_k \gets \texttt{Device\_Placement}(P_k, P_{k-1})$\;
        }
        \KwRet{$T, P$}
    \end{minipage}
    }
\end{algorithm}

==> alg_workset_selection.tex <==

\begin{algorithm}[htbp]
    \caption{Working Set Selection}
    \label{alg:workset_sel}
    \scalebox{0.92}{
    \begin{minipage}{\textwidth}
        \LinesNotNumbered
        \DontPrintSemicolon
        \While{\pqat.top.n $\leq N_{remain}$}{
                $p \gets$ \pqat.pop()\;
                \eIf{$p.m$ repeats in $\setsub{work}$}{
                    $\setsub{repeat}$.append($p$)\;
                }{
                    $\setsub{work}$.append($p$)\;
                    $N_{remain} \gets N_{remain} - p.n$\;
                }
            }
    \end{minipage}
    }
\end{algorithm}


==> append_api.tex <==
\section {Implementation Details of MTP Framework}

Our entire framework is built on PyTorch, and the communication group leverages NCCL for its underlying operations.


\subsection*{Dataloading Elimination by Task Placement}


As previously discussed, within our system, we have a unified model that is updated by multiple tasks simultaneously. Each task is characterized by distinct input and its associated activation path within the model. To optimize resource utilization, we eliminate unnecessary data loading operations that do not contribute to the computation of the first stage on a given device. This heterogeneous setup is designed to conserve CPU resources. 


\subsection*{Memory Optimization with Deferred Parameter Initialization}


In standard training routines, parameters occupy resident GPU memory. However, in our system, the required parameters are only determined after generating a plan for a given workload. Consequently, we apply a deferred initialization of model parameters, and then select some to materialize based on the plan. Our framework offers two methods. The first involves providing essential details such as the module class and arguments encapsulated in a data structure defined in our framework, enabling lazy initialization at the backend. The second method allows users to pass a regular PyTorch model, which will be initialized later using \href{https://github.com/pytorch/torchdistx}{torchdistx}. The latter option facilitates an easier migration of model training to the MTP framework with minimal additional effort for the users.

\subsection*{Automatic Splitting via Tracing}


To facilitate agile scheduling, we aim to discern the types of layers and their connections within the model. Following an extensive evaluation, we have selected the FX Tracer for creating the complete graph. Typically, the workloads we deal with are composed of homogeneous structures, like transformer layers or ResNet blocks. We refer to these layers as meta layers and meticulously schedule them, necessitating only coarse-grained granularity for effective tracing. By wrapping our meta layers, we effectively bypass complications arising from cases that are difficult to trace, which frequently pose significant challenges.

Another challenge we face pertains to the data-dependent control flow. In the context of multimodal processing, the model selects which submodule to utilize for the current input based on the input's modality or data format. Presently, the range of choices is finite and corresponds directly with the number of tasks. Therefore, we can construct dummy input specifically for each task during the tracing procedure. Consequently, for any given input, the path of control flow is precisely determined.

We integrated all these results into the MTPModel class; for each task, MTP records one splitted model which is the outcome of applying a stage splitting determined by the Planner.
In tracing mode, we automate the insertion of dataflows by parsing FX nodes. Throughout this process, we resolved numerous issues, including those related to default arguments and the order of dataflow insertion.

==> draft.tex <==

% 第一个step：构造meta op。
% 画一个小图，左边是实际op，标注type shape / 右边是meta op，缩完图的结果
% 实现一个op list到meta op list的映射，放在4.1或5.1
% 不连续，但shape/type完全一样的2种meta op
% input data & Op type same
% 大图到小图的映射
% 两个表的映射
% stage op
% 去掉p2p

% meta op 1: [op1,op3,op5]

% scalability profiler/estimator
% 为什么要去做这个事情，详细，scalability的motivation
% 






% Graph abbreviation / condensation, MetaOp construction
% Scalability Estimator/Profiler
% Problem definition & Resource Allocator
% Scheduler / Stage Map 
% Device Placement

% 问题定义：以op为粒度，而非metaop，优化目标是给每个op分配卡数，最小化总计算时长
% metaop和scaling curve绑定，需要curve的时候才用到metaop概念，定义问题时用op，6.2需要描述如何定义问题、如何map到malleable task的问题上解。allocate和schedule分成两个subsection

% runtime engine可以拆成一个单独的section，implementation可以合在一起

% 图里的文字放到caption里

% 不需要stageop，可以留stage概念，stagegraph代替stageop



% 需要做的改动

% 从实数点shift到两个离散点，不影响optimal的性质，这点需要更多解释？在工作量上和总工作时间上能线性表出
% Stage scheduler开头，stage的定义，stage的motivation和管理资源的模式，stage是scheduler过程中产生的东西，代表一段时间内mtp对资源分配的管理
% problem formulation可以考虑删掉？或拿到前面？
% Graph clustering => graph contraction
% allocator差一张图
% ofasys的图太简单，更新

% 1-4章 % task概念
% modality fusion的方式改成training objective？
% 需要说明multi-task multi-modality的关系
% motivation，对异构负载的处理，画一个multi-task训练硬件利用率的时序图
% 和job scheduling的差异和关系？
% 第四章rewrite，mtp的
% speedup function加一些citation
% 和其他并行的关系，可以考虑在runtime加进去，与其他并行技术正交，前面弱化其他并行
% Algorithm里符号太多 太难懂

% abstract planner的作用是什么？不用介绍具体模块，user-friendly API，
% 架构图可以考虑放到最前面？
% 架构图里放一些缩略图进去
% GPU cluster怎么处理？可以和tasks作为一个简单的输入
% stage map图里编号可以考虑抹掉



% framework图画法调整，需要中间结果的缩略图
% case study? 每个metaop占资源量？

% observation motivation
% 异构性展示?异构性表/图

% main body / method部分，图&文字&用词 公式需要调整




各章节名称和组件名称
5: Execution Planner
system overview和框架图直接
5.1: Graph Contraction -> MetaGraph
5.2: Scalability Estimator -> Scaling Curves
5.3: Resource Allocator -> Allocation Plan
5.4: Stage Scheduler -> Stage-level Schedule
5.5: Device Placement -> Excution Plan (Figure 5中名称，弃用stage map,5.4 5.5共同ref figure 5）

6: Training FrameWork
- Runtime Engine

Execution Planner和Training FrameWork在框架图上可以拆开，但section 6可以直接放到section 5的5.6里

1. 两个problem formulation放到5.1 Graph Contraction的前和后，缩图后的图改名MetaGraph
2. Allocator里分两小节，一是malleable task CNTN连续问题的定理化的结论阐释，告诉大家malleable task的最优解的形式，写成定理，并解释为什么我们的问题能套用这个解法。第二节是Discretized Allocation（不用在标题强调bi-point，别人看不懂），并单独配单栏allocation图以及example的解释。


TODO:

intro改图

scaling curve对每个mop需要有切分维度的属性

Decoupled Resource Allocation
标卡数

dependency挪到allocator里

实验图需要修改

MetaOp p调小
改标题

尽量图片字号比figure 3大

3.3挪到后面related work

device placement memory bound




WYJ TODO:
intro模型结构图 ok
缩preliminary and related work  ok
scheduler改成举例子 ok
check实验文字表述 ok
dependency、level 挪到allocator前 ok
scaling curve考虑对每个mop不同切分方式做不同的建模，并ref megatron/galvatron等自动并行文章的建模 ok

加reference  ok


estimator
scheduler
placement
